Attention Mechanism based Cognition-level Scene Understanding

Given a question-image input, the Visual Commonsense Reasoning (VCR) model can predict an answer with the corresponding rationale, which requires inference ability from the real world. The VCR task, which calls for exploiting the multi-source information as well as learning different levels of understanding and extensive commonsense knowledge, is a cognition-level scene understanding task. The VCR task has aroused researchers' interest due to its wide range of applications, including visual question answering, automated vehicle systems, and clinical decision support. Previous approaches to solving the VCR task generally rely on pre-training or exploiting memory with long dependency relationship encoded models. However, these approaches suffer from a lack of generalizability and losing information in long sequences. In this paper, we propose a parallel attention-based cognitive VCR network PAVCR, which fuses visual-textual information efficiently and encodes semantic information in parallel to enable the model to capture rich information for cognition-level inference. Extensive experiments show that the proposed model yields significant improvements over existing methods on the benchmark VCR dataset. Moreover, the proposed model provides intuitive interpretation into visual commonsense reasoning.

==> Definitions/journalnames.tex <==
% Updated 17 December 2024 used in Y2025
%% --------------------------------------------------------------------
%\DeclareOption{}{%
%	\gdef\@journal{}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalfull: Journal full name
%% - @journalshort: Short Name (ISO4)
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.3390/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{accountaudit}{%
        \gdef\@journal{accountaudit}
        \gdef\@journalfull{Accounting and Auditing}
        \gdef\@journalshort{Account. Audit.}
        \gdef\@doiabbr{accountaudit}
        \gdef\@ISSN{}        
        \gdef\@societyowner{}
}
\DeclareOption{acoustics}{%
	\gdef\@journal{acoustics}
	\gdef\@journalfull{Acoustics}
	\gdef\@journalshort{Acoustics}
	\gdef\@doiabbr{acoustics}
	\gdef\@ISSN{2624-599X}	
	\gdef\@societyowner{}
}
\DeclareOption{actuators}{%
	\gdef\@journal{actuators}
	\gdef\@journalfull{Actuators}
	\gdef\@journalshort{Actuators}
	\gdef\@doiabbr{act}
	\gdef\@ISSN{2076-0825}
	\gdef\@societyowner{}
}
\DeclareOption{addictions}{%
	\gdef\@journal{addictions}
	\gdef\@journalfull{Addictions}
	\gdef\@journalshort{Addictions}
	\gdef\@doiabbr{addictions}
	\gdef\@ISSN{0006-0006}
	\gdef\@societyowner{}
}
\DeclareOption{adhesives}{%
	\gdef\@journal{adhesives}
	\gdef\@journalfull{Adhesives}
	\gdef\@journalshort{Adhesives}
	\gdef\@doiabbr{adhesives}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{admsci}{%
	\gdef\@journal{admsci}
	\gdef\@journalfull{Administrative Sciences}
	\gdef\@journalshort{Adm. Sci.}
	\gdef\@doiabbr{admsci}
	\gdef\@ISSN{2076-3387}
	\gdef\@societyowner{}
}
\DeclareOption{adolescents}{%
	\gdef\@journal{adolescents}
	\gdef\@journalfull{Adolescents}
	\gdef\@journalshort{Adolescents}
	\gdef\@doiabbr{adolescents}
	\gdef\@ISSN{2673-7051}	
	\gdef\@societyowner{}
}
\DeclareOption{aerobiology}{%
	\gdef\@journal{aerobiology}
	\gdef\@journalfull{Aerobiology}
	\gdef\@journalshort{Aerobiology}
	\gdef\@doiabbr{aerobiology}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{aerospace}{%
	\gdef\@journal{aerospace}
	\gdef\@journalfull{Aerospace}
	\gdef\@journalshort{Aerospace}
	\gdef\@doiabbr{aerospace}
	\gdef\@ISSN{2226-4310}
	\gdef\@societyowner{}
}
\DeclareOption{agriculture}{%
	\gdef\@journal{agriculture}
	\gdef\@journalfull{Agriculture}
	\gdef\@journalshort{Agriculture}
	\gdef\@doiabbr{agriculture}
	\gdef\@ISSN{2077-0472}
	\gdef\@societyowner{}
}
\DeclareOption{agriengineering}{%
	\gdef\@journal{agriengineering}
	\gdef\@journalfull{AgriEngineering}
	\gdef\@journalshort{AgriEngineering}
	\gdef\@doiabbr{agriengineering}
	\gdef\@ISSN{2624-7402}	
	\gdef\@societyowner{}
}
\DeclareOption{agrochemicals}{%
	\gdef\@journal{agrochemicals}
	\gdef\@journalfull{Agrochemicals}
	\gdef\@journalshort{Agrochemicals}
	\gdef\@doiabbr{agrochemicals}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{agronomy}{%
	\gdef\@journal{agronomy}
	\gdef\@journalfull{Agronomy}
	\gdef\@journalshort{Agronomy}
	\gdef\@doiabbr{agronomy}
	\gdef\@ISSN{2073-4395}
	\gdef\@societyowner{}
}
\DeclareOption{ai}{%
	\gdef\@journal{ai}
	\gdef\@journalfull{AI}
	\gdef\@journalshort{AI}
	\gdef\@doiabbr{ai}
	\gdef\@ISSN{2673-2688}	
	\gdef\@societyowner{}
}
\DeclareOption{air}{%
	\gdef\@journal{air}
	\gdef\@journalfull{Air}
	\gdef\@journalshort{Air}
	\gdef\@doiabbr{air}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{algorithms}{%
	\gdef\@journal{algorithms}
	\gdef\@journalfull{Algorithms}
	\gdef\@journalshort{Algorithms}
	\gdef\@doiabbr{a}
	\gdef\@ISSN{1999-4893}
	\gdef\@societyowner{}
}
\DeclareOption{allergies}{%
	\gdef\@journal{allergies}
	\gdef\@journalfull{Allergies}
	\gdef\@journalshort{Allergies}
	\gdef\@doiabbr{allergies}
	\gdef\@ISSN{2313-5786}	
	\gdef\@societyowner{}
}
\DeclareOption{alloys}{%
	\gdef\@journal{alloys}
	\gdef\@journalfull{Alloys}
	\gdef\@journalshort{Alloys}
	\gdef\@doiabbr{alloys}
	\gdef\@ISSN{2674-063X}	
	\gdef\@societyowner{}
}
\DeclareOption{amh}{%
	\gdef\@journal{amh}
	\gdef\@journalfull{Acta Microbiologica Hellenica}
	\gdef\@journalshort{Acta Microbiol. Hell.}
	\gdef\@doiabbr{amh}
	\gdef\@ISSN{0438-9573}	
	\gdef\@societyowner{Hellenic Society for Microbiology}
}
\DeclareOption{analytica}{%
	\gdef\@journal{analytica}
	\gdef\@journalfull{Analytica}
	\gdef\@journalshort{Analytica}
	\gdef\@doiabbr{analytica}
	\gdef\@ISSN{2673-4532}	
	\gdef\@societyowner{}
}
\DeclareOption{analytics}{%
	\gdef\@journal{analytics}
	\gdef\@journalfull{Analytics}
	\gdef\@journalshort{Analytics}
	\gdef\@doiabbr{analytics}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{anatomia}{%
	\gdef\@journal{anatomia}
	\gdef\@journalfull{Anatomia}
	\gdef\@journalshort{Anatomia}
	\gdef\@doiabbr{anatomia}
	\gdef\@ISSN{2813-0545}	
	\gdef\@societyowner{}
}
\DeclareOption{anesthres}{%
	\gdef\@journal{anesthres}
	\gdef\@journalfull{Anesthesia Research}
	\gdef\@journalshort{Anesth. Res.}
	\gdef\@doiabbr{anesthres}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{animals}{%
	\gdef\@journal{animals}
	\gdef\@journalfull{Animals}
	\gdef\@journalshort{Animals}
	\gdef\@doiabbr{ani}
	\gdef\@ISSN{2076-2615}
	\gdef\@societyowner{}
}
\DeclareOption{antibiotics}{%
	\gdef\@journal{antibiotics}
	\gdef\@journalfull{Antibiotics}
	\gdef\@journalshort{Antibiotics}
	\gdef\@doiabbr{antibiotics}
	\gdef\@ISSN{2079-6382}
	\gdef\@societyowner{}
}
\DeclareOption{antibodies}{%
	\gdef\@journal{antibodies}
	\gdef\@journalfull{Antibodies}
	\gdef\@journalshort{Antibodies}
	\gdef\@doiabbr{antib}
	\gdef\@ISSN{2073-4468}
	\gdef\@societyowner{}
}
\DeclareOption{antioxidants}{%
	\gdef\@journal{antioxidants}
	\gdef\@journalfull{Antioxidants}
	\gdef\@journalshort{Antioxidants}
	\gdef\@doiabbr{antiox}
	\gdef\@ISSN{2076-3921}
	\gdef\@societyowner{}
}
\DeclareOption{applbiosci}{%
	\gdef\@journal{applbiosci}
	\gdef\@journalfull{Applied Biosciences}
	\gdef\@journalshort{Appl. Biosci.}
	\gdef\@doiabbr{applbiosci}
	\gdef\@ISSN{2813-0464}	
	\gdef\@societyowner{}
}
\DeclareOption{appliedchem}{%
	\gdef\@journal{appliedchem}
	\gdef\@journalfull{AppliedChem}
	\gdef\@journalshort{AppliedChem}
	\gdef\@doiabbr{appliedchem}
	\gdef\@ISSN{2673-9623}	
	\gdef\@societyowner{}
}
\DeclareOption{appliedmath}{%
	\gdef\@journal{appliedmath}
	\gdef\@journalfull{AppliedMath}
	\gdef\@journalshort{AppliedMath}
	\gdef\@doiabbr{appliedmath}
	\gdef\@ISSN{2673-9909}	
	\gdef\@societyowner{}
}
\DeclareOption{appliedphys}{%
	\gdef\@journal{appliedphys}
	\gdef\@journalfull{AppliedPhys}
	\gdef\@journalshort{AppliedPhys}
	\gdef\@doiabbr{appliedphys}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{applmech}{%
	\gdef\@journal{applmech}
	\gdef\@journalfull{Applied Mechanics}
	\gdef\@journalshort{Appl. Mech.}
	\gdef\@doiabbr{applmech}
	\gdef\@ISSN{2673-3161}	
	\gdef\@societyowner{}
}
\DeclareOption{applmicrobiol}{%
	\gdef\@journal{applmicrobiol}
	\gdef\@journalfull{Applied Microbiology}
	\gdef\@journalshort{Appl. Microbiol.}
	\gdef\@doiabbr{applmicrobiol}
	\gdef\@ISSN{2673-8007}	
	\gdef\@societyowner{}
}
\DeclareOption{applnano}{%
	\gdef\@journal{applnano}
	\gdef\@journalfull{Applied Nano}
	\gdef\@journalshort{Appl. Nano}
	\gdef\@doiabbr{applnano}
	\gdef\@ISSN{2673-3501}	
	\gdef\@societyowner{}
}
\DeclareOption{applsci}{%
	\gdef\@journal{applsci}
	\gdef\@journalfull{Applied Sciences}
	\gdef\@journalshort{Appl. Sci.}
	\gdef\@doiabbr{app}
	\gdef\@ISSN{2076-3417}
	\gdef\@societyowner{}
}
\DeclareOption{aquacj}{%
	\gdef\@journal{aquacj}
	\gdef\@journalfull{Aquaculture Journal}
	\gdef\@journalshort{Aquac. J.}
	\gdef\@doiabbr{aquacj}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{architecture}{%
	\gdef\@journal{architecture}
	\gdef\@journalfull{Architecture}
	\gdef\@journalshort{Architecture}
	\gdef\@doiabbr{architecture}
	\gdef\@ISSN{2673-8945}	
	\gdef\@societyowner{}
}
\DeclareOption{arm}{%
	\gdef\@journal{arm}
	\gdef\@journalfull{Advances in Respiratory Medicine}
	\gdef\@journalshort{Adv. Respir. Med.}
	\gdef\@doiabbr{arm}
	\gdef\@ISSN{2543-6031}	
	\gdef\@societyowner{Polish Respiratory Society}
}
\DeclareOption{arthropoda}{%
	\gdef\@journal{arthropoda}
	\gdef\@journalfull{Arthropoda}
	\gdef\@journalshort{Arthropoda}
	\gdef\@doiabbr{arthropoda}
	\gdef\@ISSN{2813-3323}	
	\gdef\@societyowner{}
}
\DeclareOption{arts}{%
	\gdef\@journal{arts}
	\gdef\@journalfull{Arts}
	\gdef\@journalshort{Arts}
	\gdef\@doiabbr{arts}
	\gdef\@ISSN{2076-0752}
	\gdef\@societyowner{}
}
\DeclareOption{asc}{%
	\gdef\@journal{asc}
	\gdef\@journalfull{Automatic Systems and Control}
	\gdef\@journalshort{Autom. Syst. Control}
	\gdef\@doiabbr{asc}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{asi}{%
	\gdef\@journal{asi}
	\gdef\@journalfull{Applied System Innovation}
	\gdef\@journalshort{Appl. Syst. Innov.}
	\gdef\@doiabbr{asi}
	\gdef\@ISSN{2571-5577}
	\gdef\@societyowner{International Institute of Knowledge Innovation and Invention}
}
\DeclareOption{astronomy}{%
	\gdef\@journal{astronomy}
	\gdef\@journalfull{Astronomy}
	\gdef\@journalshort{Astronomy}
	\gdef\@doiabbr{astronomy}
	\gdef\@ISSN{2674-0346}	
	\gdef\@societyowner{}
}
\DeclareOption{atmosphere}{%
	\gdef\@journal{atmosphere}
	\gdef\@journalfull{Atmosphere}
	\gdef\@journalshort{Atmosphere}
	\gdef\@doiabbr{atmos}
	\gdef\@ISSN{2073-4433}
	\gdef\@societyowner{}
}
\DeclareOption{atoms}{%
	\gdef\@journal{atoms}
	\gdef\@journalfull{Atoms}
	\gdef\@journalshort{Atoms}
	\gdef\@doiabbr{atoms}
	\gdef\@ISSN{2218-2004}
	\gdef\@societyowner{}
}
\DeclareOption{audiolres}{%
	\gdef\@journal{audiolres}
	\gdef\@journalfull{Audiology Research}
	\gdef\@journalshort{Audiol. Res.}
	\gdef\@doiabbr{audiolres}
	\gdef\@ISSN{2039-4349}	
	\gdef\@societyowner{}
}
\DeclareOption{automation}{%
	\gdef\@journal{automation}
	\gdef\@journalfull{Automation}
	\gdef\@journalshort{Automation}
	\gdef\@doiabbr{automation}
	\gdef\@ISSN{2673-4052}	
	\gdef\@societyowner{}
}
\DeclareOption{axioms}{%
	\gdef\@journal{axioms}
	\gdef\@journalfull{Axioms}
	\gdef\@journalshort{Axioms}
	\gdef\@doiabbr{axioms}
	\gdef\@ISSN{2075-1680}
	\gdef\@societyowner{}
}
\DeclareOption{bacteria}{%
	\gdef\@journal{bacteria}
	\gdef\@journalfull{Bacteria}
	\gdef\@journalshort{Bacteria}
	\gdef\@doiabbr{bacteria}
	\gdef\@ISSN{2674-1334}	
	\gdef\@societyowner{}
}
\DeclareOption{batteries}{%
	\gdef\@journal{batteries}
	\gdef\@journalfull{Batteries}
	\gdef\@journalshort{Batteries}
	\gdef\@doiabbr{batteries}
	\gdef\@ISSN{2313-0105}
	\gdef\@societyowner{}
}
\DeclareOption{bdcc}{%
	\gdef\@journal{bdcc}
	\gdef\@journalfull{Big Data and Cognitive Computing}
	\gdef\@journalshort{Big Data Cogn. Comput.}
	\gdef\@doiabbr{bdcc}
	\gdef\@ISSN{2504-2289}
	\gdef\@societyowner{}
}
\DeclareOption{behavsci}{%
	\gdef\@journal{behavsci}
	\gdef\@journalfull{Behavioral Sciences}
	\gdef\@journalshort{Behav. Sci.}
	\gdef\@doiabbr{bs}
	\gdef\@ISSN{2076-328X}
	\gdef\@societyowner{}
}
\DeclareOption{beverages}{%
	\gdef\@journal{beverages}
	\gdef\@journalfull{Beverages}
	\gdef\@journalshort{Beverages}
	\gdef\@doiabbr{beverages}
	\gdef\@ISSN{2306-5710}
	\gdef\@societyowner{}
}
\DeclareOption{biochem}{%
	\gdef\@journal{biochem}
	\gdef\@journalfull{BioChem}
	\gdef\@journalshort{BioChem}
	\gdef\@doiabbr{biochem}
	\gdef\@ISSN{2673-6411}	
	\gdef\@societyowner{}
}
\DeclareOption{bioengineering}{%
	\gdef\@journal{bioengineering}
	\gdef\@journalfull{Bioengineering}
	\gdef\@journalshort{Bioengineering}
	\gdef\@doiabbr{bioengineering}
	\gdef\@ISSN{2306-5354}
	\gdef\@societyowner{}
}
\DeclareOption{biologics}{%
	\gdef\@journal{biologics}
	\gdef\@journalfull{Biologics}
	\gdef\@journalshort{Biologics}
	\gdef\@doiabbr{biologics}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{biology}{%
	\gdef\@journal{biology}
	\gdef\@journalfull{Biology}
	\gdef\@journalshort{Biology}
	\gdef\@doiabbr{biology}
	\gdef\@ISSN{2079-7737}
	\gdef\@societyowner{}
}
\DeclareOption{biomass}{%
	\gdef\@journal{biomass}
	\gdef\@journalfull{Biomass}
	\gdef\@journalshort{Biomass}
	\gdef\@doiabbr{biomass}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{biomechanics}{%
	\gdef\@journal{biomechanics}
	\gdef\@journalfull{Biomechanics}
	\gdef\@journalshort{Biomechanics}
	\gdef\@doiabbr{biomechanics}
	\gdef\@ISSN{2673-7078}	
	\gdef\@societyowner{}
}
\DeclareOption{biomed}{%
	\gdef\@journal{biomed}
	\gdef\@journalfull{BioMed}
	\gdef\@journalshort{BioMed}
	\gdef\@doiabbr{biomed}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{biomedicines}{%
	\gdef\@journal{biomedicines}
	\gdef\@journalfull{Biomedicines}
	\gdef\@journalshort{Biomedicines}
	\gdef\@doiabbr{biomedicines}
	\gdef\@ISSN{2227-9059}
	\gdef\@societyowner{}
}
\DeclareOption{biomedinformatics}{%
	\gdef\@journal{biomedinformatics}
	\gdef\@journalfull{BioMedInformatics}
	\gdef\@journalshort{BioMedInformatics}
	\gdef\@doiabbr{biomedinformatics}
	\gdef\@ISSN{2673-7426}	
	\gdef\@societyowner{}
}
\DeclareOption{biomimetics}{%
	\gdef\@journal{biomimetics}
	\gdef\@journalfull{Biomimetics}
	\gdef\@journalshort{Biomimetics}
	\gdef\@doiabbr{biomimetics}
	\gdef\@ISSN{2313-7673}
	\gdef\@societyowner{}
}
\DeclareOption{biomolecules}{%
	\gdef\@journal{biomolecules}
	\gdef\@journalfull{Biomolecules}
	\gdef\@journalshort{Biomolecules}
	\gdef\@doiabbr{biom}
	\gdef\@ISSN{2218-273X}
	\gdef\@societyowner{}
}
\DeclareOption{biophysica}{%
	\gdef\@journal{biophysica}
	\gdef\@journalfull{Biophysica}
	\gdef\@journalshort{Biophysica}
	\gdef\@doiabbr{biophysica}
	\gdef\@ISSN{2673-4125}	
	\gdef\@societyowner{}
}
\DeclareOption{biosensors}{%
	\gdef\@journal{biosensors}
	\gdef\@journalfull{Biosensors}
	\gdef\@journalshort{Biosensors}
	\gdef\@doiabbr{bios}
	\gdef\@ISSN{2079-6374}
	\gdef\@societyowner{}
}
\DeclareOption{biosphere}{%
       \gdef\@journal{biosphere}
       \gdef\@journalfull{Biosphere}
       \gdef\@journalshort{Biosphere}
       \gdef\@doiabbr{biosphere}
       \gdef\@ISSN{}
       \gdef\@societyowner{}
}
\DeclareOption{biotech}{%
	\gdef\@journal{biotech}
	\gdef\@journalfull{BioTech}
	\gdef\@journalshort{BioTech}
	\gdef\@doiabbr{biotech}
	\gdef\@ISSN{2673-6284}
	\gdef\@societyowner{}
}
\DeclareOption{birds}{%
	\gdef\@journal{birds}
	\gdef\@journalfull{Birds}
	\gdef\@journalshort{Birds}
	\gdef\@doiabbr{birds}
	\gdef\@ISSN{2673-6004}	
	\gdef\@societyowner{}
}
\DeclareOption{blockchains}{%
	\gdef\@journal{blockchains}
	\gdef\@journalfull{Blockchains}
	\gdef\@journalshort{Blockchains}
	\gdef\@doiabbr{blockchains}
	\gdef\@ISSN{2813-5288}	
	\gdef\@societyowner{}
}
\DeclareOption{bloods}{%
	\gdef\@journal{bloods}
	\gdef\@journalfull{Bloods}
	\gdef\@journalshort{Bloods}
	\gdef\@doiabbr{bloods}
	\gdef\@ISSN{2673-415X}
	\gdef\@societyowner{}
}
\DeclareOption{blsf}{%
	\gdef\@journal{blsf}
	\gdef\@journalfull{Biology and Life Sciences Forum}
	\gdef\@journalshort{Biol. Life Sci. Forum}
	\gdef\@doiabbr{blsf}
	\gdef\@ISSN{2673-9976}
	\gdef\@societyowner{}
}
\DeclareOption{brainsci}{%
	\gdef\@journal{brainsci}
	\gdef\@journalfull{Brain Sciences}
	\gdef\@journalshort{Brain Sci.}
	\gdef\@doiabbr{brainsci}
	\gdef\@ISSN{2076-3425}
	\gdef\@societyowner{}
}
\DeclareOption{breath}{%
	\gdef\@journal{breath}
	\gdef\@journalfull{Breath}
	\gdef\@journalshort{Breath}
	\gdef\@doiabbr{breath}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{buildings}{%
	\gdef\@journal{buildings}
	\gdef\@journalfull{Buildings}
	\gdef\@journalshort{Buildings}
	\gdef\@doiabbr{buildings}
	\gdef\@ISSN{2075-5309}
	\gdef\@societyowner{}
}
\DeclareOption{businesses}{%
	\gdef\@journal{businesses}
	\gdef\@journalfull{Businesses}
	\gdef\@journalshort{Businesses}
	\gdef\@doiabbr{businesses}
	\gdef\@ISSN{2673-7116}	
	\gdef\@societyowner{}
}
\DeclareOption{cancers}{%
	\gdef\@journal{cancers}
	\gdef\@journalfull{Cancers}
	\gdef\@journalshort{Cancers}
	\gdef\@doiabbr{cancers}
	\gdef\@ISSN{2072-6694}
	\gdef\@societyowner{}
}
\DeclareOption{carbon}{%
	\gdef\@journal{carbon}
	\gdef\@journalfull{C}
	\gdef\@journalshort{C}
	\gdef\@doiabbr{c}
	\gdef\@ISSN{2311-5629}
	\gdef\@societyowner{}
}
\DeclareOption{cardiogenetics}{%
	\gdef\@journal{cardiogenetics}
	\gdef\@journalfull{Cardiogenetics}
	\gdef\@journalshort{Cardiogenetics}
	\gdef\@doiabbr{cardiogenetics}
	\gdef\@ISSN{2035-8148}	
	\gdef\@societyowner{}
}
\DeclareOption{catalysts}{%
	\gdef\@journal{catalysts}
	\gdef\@journalfull{Catalysts}
	\gdef\@journalshort{Catalysts}
	\gdef\@doiabbr{catal}
	\gdef\@ISSN{2073-4344}
	\gdef\@societyowner{}
}
\DeclareOption{cells}{%
	\gdef\@journal{cells}
	\gdef\@journalfull{Cells}
	\gdef\@journalshort{Cells}
	\gdef\@doiabbr{cells}
	\gdef\@ISSN{2073-4409}
	\gdef\@societyowner{}
}
\DeclareOption{ceramics}{%
	\gdef\@journal{ceramics}
	\gdef\@journalfull{Ceramics}
	\gdef\@journalshort{Ceramics}
	\gdef\@doiabbr{ceramics}
	\gdef\@ISSN{2571-6131}	
	\gdef\@societyowner{}
}
\DeclareOption{challenges}{%
	\gdef\@journal{challenges}
	\gdef\@journalfull{Challenges}
	\gdef\@journalshort{Challenges}
	\gdef\@doiabbr{challe}
	\gdef\@ISSN{2078-1547}
	\gdef\@societyowner{}
}
\DeclareOption{chemengineering}{%
	\gdef\@journal{chemengineering}
	\gdef\@journalfull{ChemEngineering}
	\gdef\@journalshort{ChemEngineering}
	\gdef\@doiabbr{chemengineering}
	\gdef\@ISSN{2305-7084}
	\gdef\@societyowner{}
}
\DeclareOption{chemistry}{%
	\gdef\@journal{chemistry}
	\gdef\@journalfull{Chemistry}
	\gdef\@journalshort{Chemistry}
	\gdef\@doiabbr{chemistry}
	\gdef\@ISSN{2624-8549}	
	\gdef\@societyowner{}
}
\DeclareOption{chemosensors}{%
	\gdef\@journal{chemosensors}
	\gdef\@journalfull{Chemosensors}
	\gdef\@journalshort{Chemosensors}
	\gdef\@doiabbr{chemosensors}
	\gdef\@ISSN{2227-9040}
	\gdef\@societyowner{}
}
\DeclareOption{chemproc}{%
	\gdef\@journal{chemproc}
	\gdef\@journalfull{Chemistry Proceedings}
	\gdef\@journalshort{Chem. Proc.}
	\gdef\@doiabbr{chemproc}
	\gdef\@ISSN{2673-4583}
	\gdef\@societyowner{}
}
\DeclareOption{children}{%
	\gdef\@journal{children}
	\gdef\@journalfull{Children}
	\gdef\@journalshort{Children}
	\gdef\@doiabbr{children}
	\gdef\@ISSN{2227-9067}
	\gdef\@societyowner{}
}
\DeclareOption{chips}{%
	\gdef\@journal{chips}
	\gdef\@journalfull{Chips}
	\gdef\@journalshort{Chips}
	\gdef\@doiabbr{chips}
	\gdef\@ISSN{2674-0729}	
	\gdef\@societyowner{}
}
\DeclareOption{cimb}{%
	\gdef\@journal{cimb}
	\gdef\@journalfull{Current Issues in Molecular Biology}
	\gdef\@journalshort{Curr. Issues Mol. Biol.}
	\gdef\@doiabbr{cimb}
	\gdef\@ISSN{1467-3045}	
	\gdef\@societyowner{}
}
\DeclareOption{civileng}{%
	\gdef\@journal{civileng}
	\gdef\@journalfull{CivilEng}
	\gdef\@journalshort{CivilEng}
	\gdef\@doiabbr{civileng}
	\gdef\@ISSN{2673-4109}	
	\gdef\@societyowner{}
}
\DeclareOption{cleantechnol}{%
	\gdef\@journal{cleantechnol}
	\gdef\@journalfull{Clean Technologies}
	\gdef\@journalshort{Clean Technol.}
	\gdef\@doiabbr{cleantechnol}
	\gdef\@ISSN{2571-8797}	
	\gdef\@societyowner{}
}
\DeclareOption{climate}{%
	\gdef\@journal{climate}
	\gdef\@journalfull{Climate}
	\gdef\@journalshort{Climate}
	\gdef\@doiabbr{cli}
	\gdef\@ISSN{2225-1154}
	\gdef\@societyowner{}
}
\DeclareOption{clinbioenerg}{%
      \gdef\@journal{clinbioenerg}
      \gdef\@journalfull{Clinical Bioenergetics}
      \gdef\@journalshort{Clin. Bioenerg.}
      \gdef\@doiabbr{clinbioenerg}
      \gdef\@ISSN{3042-5158}      	
      \gdef\@societyowner{}
}
\DeclareOption{clinpract}{%
	\gdef\@journal{clinpract}
	\gdef\@journalfull{Clinics and Practice}
	\gdef\@journalshort{Clin. Pract.}
	\gdef\@doiabbr{clinpract}
	\gdef\@ISSN{2039-7283}	
	\gdef\@societyowner{}
}
\DeclareOption{clockssleep}{%
	\gdef\@journal{clockssleep}
	\gdef\@journalfull{Clocks \& Sleep}
	\gdef\@journalshort{Clocks\&Sleep}
	\gdef\@doiabbr{clockssleep}
	\gdef\@ISSN{2624-5175}	
	\gdef\@societyowner{}
}
\DeclareOption{cmd}{%
	\gdef\@journal{cmd}
	\gdef\@journalfull{Corrosion and Materials Degradation}
	\gdef\@journalshort{Corros. Mater. Degrad.}
	\gdef\@doiabbr{cmd}
	\gdef\@ISSN{2624-5558}	
	\gdef\@societyowner{}
}
\DeclareOption{cmtr}{%
        \gdef\@journal{cmtr}
        \gdef\@journalfull{Craniomaxillofacial Trauma \& Reconstruction}
        \gdef\@journalshort{Craniomaxillofac. Trauma Reconstr.}
       \gdef\@doiabbr{cmtr}
       \gdef\@ISSN{1943-3875}       
       \gdef\@societyowner{AO Foundation}
}
\DeclareOption{coasts}{%
	\gdef\@journal{coasts}
	\gdef\@journalfull{Coasts}
	\gdef\@journalshort{Coasts}
	\gdef\@doiabbr{coasts}
	\gdef\@ISSN{2673-964X}	
	\gdef\@societyowner{}
}
\DeclareOption{coatings}{%
	\gdef\@journal{coatings}
	\gdef\@journalfull{Coatings}
	\gdef\@journalshort{Coatings}
	\gdef\@doiabbr{coatings}
	\gdef\@ISSN{2079-6412}
	\gdef\@societyowner{}
}
\DeclareOption{colloids}{%
	\gdef\@journal{colloids}
	\gdef\@journalfull{Colloids and Interfaces}
	\gdef\@journalshort{Colloids Interfaces}
	\gdef\@doiabbr{colloids}
	\gdef\@ISSN{2504-5377}
	\gdef\@societyowner{}
}
\DeclareOption{colorants}{%
	\gdef\@journal{colorants}
	\gdef\@journalfull{Colorants}
	\gdef\@journalshort{Colorants}
	\gdef\@doiabbr{colorants}
	\gdef\@ISSN{2079-6447}	
	\gdef\@societyowner{}
}
\DeclareOption{commodities}{%
	\gdef\@journal{commodities}
	\gdef\@journalfull{Commodities}
	\gdef\@journalshort{Commodities}
	\gdef\@doiabbr{commodities}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{complications}{%
       \gdef\@journal{complications}
       \gdef\@journalfull{Complications}
       \gdef\@journalshort{Complications}
       \gdef\@doiabbr{complications}
       \gdef\@ISSN{}       
       \gdef\@societyowner{}
}
\DeclareOption{compounds}{%
	\gdef\@journal{compounds}
	\gdef\@journalfull{Compounds}
	\gdef\@journalshort{Compounds}
	\gdef\@doiabbr{compounds}
	\gdef\@ISSN{2673-6918}	
	\gdef\@societyowner{}
}
\DeclareOption{computation}{%
	\gdef\@journal{computation}
	\gdef\@journalfull{Computation}
	\gdef\@journalshort{Computation}
	\gdef\@doiabbr{computation}
	\gdef\@ISSN{2079-3197}
	\gdef\@societyowner{}
}
\DeclareOption{computers}{%
	\gdef\@journal{computers}
	\gdef\@journalfull{Computers}
	\gdef\@journalshort{Computers}
	\gdef\@doiabbr{computers}
	\gdef\@ISSN{2073-431X}
	\gdef\@societyowner{}
}
\DeclareOption{condensedmatter}{%
	\gdef\@journal{condensedmatter}
	\gdef\@journalfull{Condensed Matter}
	\gdef\@journalshort{Condens. Matter}
	\gdef\@doiabbr{condmat}
	\gdef\@ISSN{2410-3896}
	\gdef\@societyowner{}
}
\DeclareOption{conservation}{%
	\gdef\@journal{conservation}
	\gdef\@journalfull{Conservation}
	\gdef\@journalshort{Conservation}
	\gdef\@doiabbr{conservation}
	\gdef\@ISSN{2673-7159}	
	\gdef\@societyowner{}
}
\DeclareOption{constrmater}{%
	\gdef\@journal{constrmater}
	\gdef\@journalfull{Construction Materials}
	\gdef\@journalshort{Constr. Mater.}
	\gdef\@doiabbr{constrmater}
	\gdef\@ISSN{2673-7108}	
	\gdef\@societyowner{}
}
\DeclareOption{cosmetics}{%
	\gdef\@journal{cosmetics}
	\gdef\@journalfull{Cosmetics}
	\gdef\@journalshort{Cosmetics}
	\gdef\@doiabbr{cosmetics}
	\gdef\@ISSN{2079-9284}
	\gdef\@societyowner{}
}
\DeclareOption{covid}{%
	\gdef\@journal{covid}
	\gdef\@journalfull{COVID}
	\gdef\@journalshort{COVID}
	\gdef\@doiabbr{covid}
	\gdef\@ISSN{2673-8112}	
	\gdef\@societyowner{}
}
\DeclareOption{crops}{%
	\gdef\@journal{crops}
	\gdef\@journalfull{Crops}
	\gdef\@journalshort{Crops}
	\gdef\@doiabbr{crops}
	\gdef\@ISSN{2673-7655}	
	\gdef\@societyowner{}
}
\DeclareOption{cryo}{%
	\gdef\@journal{cryo}
	\gdef\@journalfull{Cryo}
	\gdef\@journalshort{Cryo}
	\gdef\@doiabbr{cryo}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{cryptography}{%
	\gdef\@journal{cryptography}
	\gdef\@journalfull{Cryptography}
	\gdef\@journalshort{Cryptography}
	\gdef\@doiabbr{cryptography}
	\gdef\@ISSN{2410-387X}
	\gdef\@societyowner{}
}
\DeclareOption{crystals}{%
	\gdef\@journal{crystals}
	\gdef\@journalfull{Crystals}
	\gdef\@journalshort{Crystals}
	\gdef\@doiabbr{cryst}
	\gdef\@ISSN{2073-4352}
	\gdef\@societyowner{}
}
\DeclareOption{csmf}{%
	\gdef\@journal{csmf}
	\gdef\@journalfull{Computer Sciences \& Mathematics Forum}
	\gdef\@journalshort{Comput. Sci. Math. Forum}
	\gdef\@doiabbr{csmf}
	\gdef\@ISSN{2813-0324}
	\gdef\@societyowner{}
}
\DeclareOption{ctn}{%
	\gdef\@journal{ctn}
	\gdef\@journalfull{Clinical and Translational Neuroscience}
	\gdef\@journalshort{Clin. Transl. Neurosci.}
	\gdef\@doiabbr{ctn}
	\gdef\@ISSN{2514-183X}
	\gdef\@societyowner{Swiss Federation of Clinical Neuro-Societies}
}
\DeclareOption{curroncol}{%
	\gdef\@journal{curroncol}
	\gdef\@journalfull{Current Oncology}
	\gdef\@journalshort{Curr. Oncol.}
	\gdef\@doiabbr{curroncol}
	\gdef\@ISSN{1718-7729}	
	\gdef\@societyowner{}
}
\DeclareOption{cyber}{%
	\gdef\@journal{cyber}
	\gdef\@journalfull{Cyber}
	\gdef\@journalshort{Cyber}
	\gdef\@doiabbr{cyber}
	\gdef\@ISSN{2624-800X}
	\gdef\@societyowner{}
}
\DeclareOption{dairy}{%
	\gdef\@journal{dairy}
	\gdef\@journalfull{Dairy}
	\gdef\@journalshort{Dairy}
	\gdef\@doiabbr{dairy}
	\gdef\@ISSN{2624-862X}	
	\gdef\@societyowner{}
}
\DeclareOption{data}{%
	\gdef\@journal{data}
	\gdef\@journalfull{Data}
	\gdef\@journalshort{Data}
	\gdef\@doiabbr{data}
	\gdef\@ISSN{2306-5729}
	\gdef\@societyowner{}
}
\DeclareOption{ddc}{%
	\gdef\@journal{ddc}
	\gdef\@journalfull{Drugs and Drug Candidates}
	\gdef\@journalshort{Drugs Drug Candidates}
	\gdef\@doiabbr{ddc}
	\gdef\@ISSN{2813-2998}	
	\gdef\@societyowner{}
}
\DeclareOption{dentistry}{%
	\gdef\@journal{dentistry}
	\gdef\@journalfull{Dentistry Journal}
	\gdef\@journalshort{Dent. J.}
	\gdef\@doiabbr{dj}
	\gdef\@ISSN{2304-6767}
	\gdef\@societyowner{}
}
\DeclareOption{dermato}{%
	\gdef\@journal{dermato}
	\gdef\@journalfull{Dermato}
	\gdef\@journalshort{Dermato}
	\gdef\@doiabbr{dermato}
	\gdef\@ISSN{2673-6179}	
	\gdef\@societyowner{}
}
\DeclareOption{dermatopathology}{%
	\gdef\@journal{dermatopathology}
	\gdef\@journalfull{Dermatopathology}
	\gdef\@journalshort{Dermatopathology}
	\gdef\@doiabbr{dermatopathology}
	\gdef\@ISSN{2296-3529}	
	\gdef\@societyowner{European Society of Dermatopathology}
}
\DeclareOption{designs}{%
	\gdef\@journal{designs}
	\gdef\@journalfull{Designs}
	\gdef\@journalshort{Designs}
	\gdef\@doiabbr{designs}
	\gdef\@ISSN{2411-9660}
	\gdef\@societyowner{}
}
\DeclareOption{devices}{%
	\gdef\@journal{devices}
	\gdef\@journalfull{Devices}
	\gdef\@journalshort{Devices}
	\gdef\@doiabbr{devices}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{diabetology}{%
	\gdef\@journal{diabetology}
	\gdef\@journalfull{Diabetology}
	\gdef\@journalshort{Diabetology}
	\gdef\@doiabbr{diabetology}
	\gdef\@ISSN{2673-4540}	
	\gdef\@societyowner{}
}
\DeclareOption{diagnostics}{%
	\gdef\@journal{diagnostics}
	\gdef\@journalfull{Diagnostics}
	\gdef\@journalshort{Diagnostics}
	\gdef\@doiabbr{diagnostics}
	\gdef\@ISSN{2075-4418}
	\gdef\@societyowner{}
}
\DeclareOption{dietetics}{%
	\gdef\@journal{dietetics}
	\gdef\@journalfull{Dietetics}
	\gdef\@journalshort{Dietetics}
	\gdef\@doiabbr{dietetics}
	\gdef\@ISSN{2674-0311}	
	\gdef\@societyowner{}
}
\DeclareOption{digital}{%
	\gdef\@journal{digital}
	\gdef\@journalfull{Digital}
	\gdef\@journalshort{Digital}
	\gdef\@doiabbr{digital}
	\gdef\@ISSN{2673-6470}	
	\gdef\@societyowner{}
}
\DeclareOption{disabilities}{%
	\gdef\@journal{disabilities}
	\gdef\@journalfull{Disabilities}
	\gdef\@journalshort{Disabilities}
	\gdef\@doiabbr{disabilities}
	\gdef\@ISSN{2673-7272}	
	\gdef\@societyowner{}
}
\DeclareOption{diseases}{%
	\gdef\@journal{diseases}
	\gdef\@journalfull{Diseases}
	\gdef\@journalshort{Diseases}
	\gdef\@doiabbr{diseases}
	\gdef\@ISSN{2079-9721}
	\gdef\@societyowner{}
}
\DeclareOption{diversity}{%
	\gdef\@journal{diversity}
	\gdef\@journalfull{Diversity}
	\gdef\@journalshort{Diversity}
	\gdef\@doiabbr{d}
	\gdef\@ISSN{1424-2818}
	\gdef\@societyowner{}
}
\DeclareOption{dna}{%
	\gdef\@journal{dna}
	\gdef\@journalfull{DNA}
	\gdef\@journalshort{DNA}
	\gdef\@doiabbr{dna}
	\gdef\@ISSN{2673-8856}	
	\gdef\@societyowner{}
}
\DeclareOption{drones}{%
	\gdef\@journal{drones}
	\gdef\@journalfull{Drones}
	\gdef\@journalshort{Drones}
	\gdef\@doiabbr{drones}
	\gdef\@ISSN{2504-446X}
	\gdef\@societyowner{}
}
\DeclareOption{dynamics}{%
	\gdef\@journal{dynamics}
	\gdef\@journalfull{Dynamics}
	\gdef\@journalshort{Dynamics}
	\gdef\@doiabbr{dynamics}
	\gdef\@ISSN{2673-8716}	
	\gdef\@societyowner{}
}
\DeclareOption{earth}{%
	\gdef\@journal{earth}
	\gdef\@journalfull{Earth}
	\gdef\@journalshort{Earth}
	\gdef\@doiabbr{earth}
	\gdef\@ISSN{2673-4834}	
	\gdef\@societyowner{}
}
\DeclareOption{ebj}{%
	\gdef\@journal{ebj}
	\gdef\@journalfull{European Burn Journal}
	\gdef\@journalshort{Eur. Burn J.}
	\gdef\@doiabbr{ebj}
	\gdef\@ISSN{2673-1991}	
	\gdef\@societyowner{European Burns Association}
}
\DeclareOption{ecm}{%
	\gdef\@journal{ecm}
	\gdef\@journalfull{Emergency Care and Medicine}
	\gdef\@journalshort{Emerg. Care Med.}
	\gdef\@doiabbr{ecm}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{ecologies}{%
	\gdef\@journal{ecologies}
	\gdef\@journalfull{Ecologies}
	\gdef\@journalshort{Ecologies}
	\gdef\@doiabbr{ecologies}
	\gdef\@ISSN{2673-4133}	
	\gdef\@societyowner{}
}
\DeclareOption{econometrics}{%
	\gdef\@journal{econometrics}
	\gdef\@journalfull{Econometrics}
	\gdef\@journalshort{Econometrics}
	\gdef\@doiabbr{econometrics}
	\gdef\@ISSN{2225-1146}
	\gdef\@societyowner{}
}
\DeclareOption{economies}{%
	\gdef\@journal{economies}
	\gdef\@journalfull{Economies}
	\gdef\@journalshort{Economies}
	\gdef\@doiabbr{economies}
	\gdef\@ISSN{2227-7099}
	\gdef\@societyowner{}
}
\DeclareOption{education}{%
	\gdef\@journal{education}
	\gdef\@journalfull{Education Sciences}
	\gdef\@journalshort{Educ. Sci.}
	\gdef\@doiabbr{educsci}
	\gdef\@ISSN{2227-7102}
	\gdef\@societyowner{}
}
\DeclareOption{ejihpe}{%
	\gdef\@journal{ejihpe}
	\gdef\@journalfull{European Journal of Investigation in Health, Psychology and Education}
	\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}
	\gdef\@doiabbr{ejihpe}
	\gdef\@ISSN{2254-9625}	
	\gdef\@societyowner{University Association of Education and Psychology}
}
\DeclareOption{electricity}{%
	\gdef\@journal{electricity}
	\gdef\@journalfull{Electricity}
	\gdef\@journalshort{Electricity}
	\gdef\@doiabbr{electricity}
	\gdef\@ISSN{2673-4826}	
	\gdef\@societyowner{}
}
\DeclareOption{electrochem}{%
	\gdef\@journal{electrochem}
	\gdef\@journalfull{Electrochem}
	\gdef\@journalshort{Electrochem}
	\gdef\@doiabbr{electrochem}
	\gdef\@ISSN{2673-3293}	
	\gdef\@societyowner{}
}
\DeclareOption{electronicmat}{%
	\gdef\@journal{electronicmat}
	\gdef\@journalfull{Electronic Materials}
	\gdef\@journalshort{Electron. Mater.}
	\gdef\@doiabbr{electronicmat}
	\gdef\@ISSN{2673-3978}	
	\gdef\@societyowner{}
}
\DeclareOption{electronics}{%
	\gdef\@journal{electronics}
	\gdef\@journalfull{Electronics}
	\gdef\@journalshort{Electronics}
	\gdef\@doiabbr{electronics}
	\gdef\@ISSN{2079-9292}
	\gdef\@societyowner{}
}
\DeclareOption{encyclopedia}{%
	\gdef\@journal{encyclopedia}
	\gdef\@journalfull{Encyclopedia}
	\gdef\@journalshort{Encyclopedia}
	\gdef\@doiabbr{encyclopedia}
	\gdef\@ISSN{2673-8392}	
	\gdef\@societyowner{}
}
\DeclareOption{endocrines}{%
	\gdef\@journal{endocrines}
	\gdef\@journalfull{Endocrines}
	\gdef\@journalshort{Endocrines}
	\gdef\@doiabbr{endocrines}
	\gdef\@ISSN{2673-396X}	
	\gdef\@societyowner{}
}
\DeclareOption{energies}{%
	\gdef\@journal{energies}
	\gdef\@journalfull{Energies}
	\gdef\@journalshort{Energies}
	\gdef\@doiabbr{en}
	\gdef\@ISSN{1996-1073}
	\gdef\@societyowner{}
}
\DeclareOption{eng}{%
	\gdef\@journal{eng}
	\gdef\@journalfull{Eng}
	\gdef\@journalshort{Eng}
	\gdef\@doiabbr{eng}
	\gdef\@ISSN{2673-4117}	
	\gdef\@societyowner{}
}
\DeclareOption{engproc}{%
	\gdef\@journal{engproc}
	\gdef\@journalfull{Engineering Proceedings}
	\gdef\@journalshort{Eng. Proc.}
	\gdef\@doiabbr{engproc}
	\gdef\@ISSN{2673-4591}
	\gdef\@societyowner{}
}
\DeclareOption{entomology}{%
	\gdef\@journal{entomology}
	\gdef\@journalfull{Entomology}
	\gdef\@journalshort{Entomology}
	\gdef\@doiabbr{entomology}
	\gdef\@ISSN{2813-0502}	
	\gdef\@societyowner{}
}
\DeclareOption{entropy}{%
	\gdef\@journal{entropy}
	\gdef\@journalfull{Entropy}
	\gdef\@journalshort{Entropy}
	\gdef\@doiabbr{e}
	\gdef\@ISSN{1099-4300}
	\gdef\@societyowner{}
}
\DeclareOption{environments}{%
	\gdef\@journal{environments}
	\gdef\@journalfull{Environments}
	\gdef\@journalshort{Environments}
	\gdef\@doiabbr{environments}
	\gdef\@ISSN{2076-3298}
	\gdef\@societyowner{}
}
\DeclareOption{eesp}{%
	\gdef\@journal{eesp}
	\gdef\@journalfull{Environmental and Earth Sciences Proceedings}
	\gdef\@journalshort{Environ. Earth Sci. Proc.}
	\gdef\@doiabbr{eesp}
	\gdef\@ISSN{3042-5743}
	\gdef\@societyowner{}
}
\DeclareOption{epidemiologia}{%
	\gdef\@journal{epidemiologia}
	\gdef\@journalfull{Epidemiologia}
	\gdef\@journalshort{Epidemiologia}
	\gdef\@doiabbr{epidemiologia}
	\gdef\@ISSN{2673-3986}	
	\gdef\@societyowner{}
}
\DeclareOption{epigenomes}{%
	\gdef\@journal{epigenomes}
	\gdef\@journalfull{Epigenomes}
	\gdef\@journalshort{Epigenomes}
	\gdef\@doiabbr{epigenomes}
	\gdef\@ISSN{2075-4655}
	\gdef\@societyowner{}
}
\DeclareOption{esa}{%
	\gdef\@journal{esa}
	\gdef\@journalfull{Energy Storage and Applications}
	\gdef\@journalshort{Energy Storage Appl.}
	\gdef\@doiabbr{esa}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{est}{%
	\gdef\@journal{est}
	\gdef\@journalfull{Electrochemical Science and Technology}
	\gdef\@journalshort{Electrochem. Sci. Technol.}
	\gdef\@doiabbr{est}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{famsci}{%
      \gdef\@journal{famsci}
      \gdef\@journalfull{Family Sciences}
      \gdef\@journalshort{Fam. Sci.}
      \gdef\@doiabbr{famsci}
      \gdef\@ISSN{}
      \gdef\@societyowner{}
}
\DeclareOption{fermentation}{%
	\gdef\@journal{fermentation}
	\gdef\@journalfull{Fermentation}
	\gdef\@journalshort{Fermentation}
	\gdef\@doiabbr{fermentation}
	\gdef\@ISSN{2311-5637}
	\gdef\@societyowner{}
}
\DeclareOption{fibers}{%
	\gdef\@journal{fibers}
	\gdef\@journalfull{Fibers}
	\gdef\@journalshort{Fibers}
	\gdef\@doiabbr{fib}
	\gdef\@ISSN{2079-6439}
	\gdef\@societyowner{}
}
\DeclareOption{fintech}{%
	\gdef\@journal{fintech}
	\gdef\@journalfull{FinTech}
	\gdef\@journalshort{FinTech}
	\gdef\@doiabbr{fintech}
	\gdef\@ISSN{2674-1032}	
	\gdef\@societyowner{}
}
\DeclareOption{fire}{%
	\gdef\@journal{fire}
	\gdef\@journalfull{Fire}
	\gdef\@journalshort{Fire}
	\gdef\@doiabbr{fire}
	\gdef\@ISSN{2571-6255}
	\gdef\@societyowner{}
}
\DeclareOption{fishes}{%
	\gdef\@journal{fishes}
	\gdef\@journalfull{Fishes}
	\gdef\@journalshort{Fishes}
	\gdef\@doiabbr{fishes}
	\gdef\@ISSN{2410-3888}
	\gdef\@societyowner{}
}
\DeclareOption{fluids}{%
	\gdef\@journal{fluids}
	\gdef\@journalfull{Fluids}
	\gdef\@journalshort{Fluids}
	\gdef\@doiabbr{fluids}
	\gdef\@ISSN{2311-5521}
	\gdef\@societyowner{}
}
\DeclareOption{foods}{%
	\gdef\@journal{foods}
	\gdef\@journalfull{Foods}
	\gdef\@journalshort{Foods}
	\gdef\@doiabbr{foods}
	\gdef\@ISSN{2304-8158}
	\gdef\@societyowner{}
}
\DeclareOption{forecasting}{%
	\gdef\@journal{forecasting}
	\gdef\@journalfull{Forecasting}
	\gdef\@journalshort{Forecasting}
	\gdef\@doiabbr{forecast}
	\gdef\@ISSN{2571-9394}	
	\gdef\@societyowner{}
}
\DeclareOption{forensicsci}{%
	\gdef\@journal{forensicsci}
	\gdef\@journalfull{Forensic Sciences}
	\gdef\@journalshort{Forensic Sci.}
	\gdef\@doiabbr{forensicsci}
	\gdef\@ISSN{2673-6756}	
	\gdef\@societyowner{}
}
\DeclareOption{forests}{%
	\gdef\@journal{forests}
	\gdef\@journalfull{Forests}
	\gdef\@journalshort{Forests}
	\gdef\@doiabbr{f}
	\gdef\@ISSN{1999-4907}
	\gdef\@societyowner{}
}
\DeclareOption{fossstud}{%
	\gdef\@journal{fossstud}
	\gdef\@journalfull{Fossil Studies}
	\gdef\@journalshort{Foss. Stud.}
	\gdef\@doiabbr{fossils}
	\gdef\@ISSN{2813-6284}	
	\gdef\@societyowner{}
}
\DeclareOption{foundations}{%
	\gdef\@journal{foundations}
	\gdef\@journalfull{Foundations}
	\gdef\@journalshort{Foundations}
	\gdef\@doiabbr{foundations}
	\gdef\@ISSN{2673-9321}	
	\gdef\@societyowner{}
}
\DeclareOption{fractalfract}{%
	\gdef\@journal{fractalfract}
	\gdef\@journalfull{Fractal and Fractional}
	\gdef\@journalshort{Fractal Fract.}
	\gdef\@doiabbr{fractalfract}
	\gdef\@ISSN{2504-3110}
	\gdef\@societyowner{}
}
\DeclareOption{fuels}{%
	\gdef\@journal{fuels}
	\gdef\@journalfull{Fuels}
	\gdef\@journalshort{Fuels}
	\gdef\@doiabbr{fuels}
	\gdef\@ISSN{2673-3994}	
	\gdef\@societyowner{}
}
\DeclareOption{future}{%
	\gdef\@journal{future}
	\gdef\@journalfull{Future}
	\gdef\@journalshort{Future}
	\gdef\@doiabbr{future}
	\gdef\@ISSN{2813-2882}	
	\gdef\@societyowner{}
}
\DeclareOption{futureinternet}{%
	\gdef\@journal{futureinternet}
	\gdef\@journalfull{Future Internet}
	\gdef\@journalshort{Future Internet}
	\gdef\@doiabbr{fi}
	\gdef\@ISSN{1999-5903}
	\gdef\@societyowner{}
}
\DeclareOption{futurepharmacol}{%
	\gdef\@journal{futurepharmacol}
	\gdef\@journalfull{Future Pharmacology}
	\gdef\@journalshort{Future Pharmacol.}
	\gdef\@doiabbr{futurepharmacol}
	\gdef\@ISSN{2673-9879}	
	\gdef\@societyowner{}
}
\DeclareOption{futurephys}{%
	\gdef\@journal{futurephys}
	\gdef\@journalfull{Future Physics}
	\gdef\@journalshort{Future Phys.}
	\gdef\@doiabbr{futurephys}
	\gdef\@ISSN{2624-6503}
	\gdef\@societyowner{}
}
\DeclareOption{futuretransp}{%
	\gdef\@journal{futuretransp}
	\gdef\@journalfull{Future Transportation}
	\gdef\@journalshort{Future Transp.}
	\gdef\@doiabbr{futuretransp}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{galaxies}{%
	\gdef\@journal{galaxies}
	\gdef\@journalfull{Galaxies}
	\gdef\@journalshort{Galaxies}
	\gdef\@doiabbr{galaxies}
	\gdef\@ISSN{2075-4434}
	\gdef\@societyowner{}
}
\DeclareOption{games}{%
	\gdef\@journal{games}
	\gdef\@journalfull{Games}
	\gdef\@journalshort{Games}
	\gdef\@doiabbr{g}
	\gdef\@ISSN{2073-4336}
	\gdef\@societyowner{}
}
\DeclareOption{gases}{%
	\gdef\@journal{gases}
	\gdef\@journalfull{Gases}
	\gdef\@journalshort{Gases}
	\gdef\@doiabbr{gases}
	\gdef\@ISSN{2673-5628}	
	\gdef\@societyowner{}
}
\DeclareOption{gastroent}{%
	\gdef\@journal{gastroent}
	\gdef\@journalfull{Gastroenterology Insights}
	\gdef\@journalshort{Gastroenterol. Insights}
	\gdef\@doiabbr{gastroent}
	\gdef\@ISSN{2036-7422}	
	\gdef\@societyowner{}
}
\DeclareOption{gastrointestdisord}{%
	\gdef\@journal{gastrointestdisord}
	\gdef\@journalfull{Gastrointestinal Disorders}
	\gdef\@journalshort{Gastrointest. Disord.}
	\gdef\@doiabbr{gidisord}
	\gdef\@ISSN{2624-5647}	
	\gdef\@societyowner{}
}
\DeclareOption{gastronomy}{%
	\gdef\@journal{gastronomy}
	\gdef\@journalfull{Gastronomy}
	\gdef\@journalshort{Gastronomy}
	\gdef\@doiabbr{gastronomy}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{gels}{%
	\gdef\@journal{gels}
	\gdef\@journalfull{Gels}
	\gdef\@journalshort{Gels}
	\gdef\@doiabbr{gels}
	\gdef\@ISSN{2310-2861}
	\gdef\@societyowner{}
}
\DeclareOption{genealogy}{%
	\gdef\@journal{genealogy}
	\gdef\@journalfull{Genealogy}
	\gdef\@journalshort{Genealogy}
	\gdef\@doiabbr{genealogy}
	\gdef\@ISSN{2313-5778}
	\gdef\@societyowner{}
}
\DeclareOption{genes}{%
	\gdef\@journal{genes}
	\gdef\@journalfull{Genes}
	\gdef\@journalshort{Genes}
	\gdef\@doiabbr{genes}
	\gdef\@ISSN{2073-4425}
	\gdef\@societyowner{}
}
\DeclareOption{geographies}{%
	\gdef\@journal{geographies}
	\gdef\@journalfull{Geographies}
	\gdef\@journalshort{Geographies}
	\gdef\@doiabbr{geographies}
	\gdef\@ISSN{2673-7086}	
	\gdef\@societyowner{}
}
\DeclareOption{geohazards}{%
	\gdef\@journal{geohazards}
	\gdef\@journalfull{GeoHazards}
	\gdef\@journalshort{GeoHazards}
	\gdef\@doiabbr{geohazards}
	\gdef\@ISSN{2624-795X}	
	\gdef\@societyowner{}
}
\DeclareOption{geomatics}{%
	\gdef\@journal{geomatics}
	\gdef\@journalfull{Geomatics}
	\gdef\@journalshort{Geomatics}
	\gdef\@doiabbr{geomatics}
	\gdef\@ISSN{2673-7418}	
	\gdef\@societyowner{}
}
\DeclareOption{geometry}{%
	\gdef\@journal{geometry}
	\gdef\@journalfull{Geometry}
	\gdef\@journalshort{Geometry}
	\gdef\@doiabbr{geometry}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{geosciences}{%
	\gdef\@journal{geosciences}
	\gdef\@journalfull{Geosciences}
	\gdef\@journalshort{Geosciences}
	\gdef\@doiabbr{geosciences}
	\gdef\@ISSN{2076-3263}
	\gdef\@societyowner{}
}
\DeclareOption{geotechnics}{%
	\gdef\@journal{geotechnics}
	\gdef\@journalfull{Geotechnics}
	\gdef\@journalshort{Geotechnics}
	\gdef\@doiabbr{geotechnics}
	\gdef\@ISSN{2673-7094}	
	\gdef\@societyowner{}
}
\DeclareOption{geriatrics}{%
	\gdef\@journal{geriatrics}
	\gdef\@journalfull{Geriatrics}
	\gdef\@journalshort{Geriatrics}
	\gdef\@doiabbr{geriatrics}
	\gdef\@ISSN{2308-3417}
	\gdef\@societyowner{}
}
\DeclareOption{glacies}{%
	\gdef\@journal{glacies}
	\gdef\@journalfull{Glacies}
	\gdef\@journalshort{Glacies}
	\gdef\@doiabbr{glacies}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{grasses}{%
	\gdef\@journal{grasses}
	\gdef\@journalfull{Grasses}
	\gdef\@journalshort{Grasses}
	\gdef\@doiabbr{grasses}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{greenhealth}{%
       \gdef\@journal{greenhealth}
       \gdef\@journalfull{Green Health}
      \gdef\@journalshort{Green Health}
      \gdef\@doiabbr{greenhealth}
      \gdef\@ISSN{}
      \gdef\@societyowner{}
}
\DeclareOption{gucdd}{%
	\gdef\@journal{gucdd}
	\gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}
	\gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}
	\gdef\@doiabbr{gucdd}
	\gdef\@ISSN{}	
	\gdef\@societyowner{Gout, Hyperuricemia and Crystal Associated Disease Network}
}
\DeclareOption{hardware}{%
	\gdef\@journal{hardware}
	\gdef\@journalfull{Hardware}
	\gdef\@journalshort{Hardware}
	\gdef\@doiabbr{hardware}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{hazardousmatters}{%
	\gdef\@journal{hazardousmatters}
	\gdef\@journalfull{Hazardous Matters}
	\gdef\@journalshort{Hazard. Matters}
	\gdef\@doiabbr{hazardousmatters}
	\gdef\@ISSN{0014-0014}
	\gdef\@societyowner{}
}
\DeclareOption{healthcare}{%
	\gdef\@journal{healthcare}
	\gdef\@journalfull{Healthcare}
	\gdef\@journalshort{Healthcare}
	\gdef\@doiabbr{healthcare}
	\gdef\@ISSN{2227-9032}
	\gdef\@societyowner{}
}
\DeclareOption{hearts}{%
	\gdef\@journal{hearts}
	\gdef\@journalfull{Hearts}
	\gdef\@journalshort{Hearts}
	\gdef\@doiabbr{hearts}
	\gdef\@ISSN{2673-3846}	
	\gdef\@societyowner{}
}
\DeclareOption{hemato}{%
	\gdef\@journal{hemato}
	\gdef\@journalfull{Hemato}
	\gdef\@journalshort{Hemato}
	\gdef\@doiabbr{hemato}
	\gdef\@ISSN{2673-6357}	
	\gdef\@societyowner{}
}
\DeclareOption{hematolrep}{%
	\gdef\@journal{hematolrep}
	\gdef\@journalfull{Hematology Reports}
	\gdef\@journalshort{Hematol. Rep.}
	\gdef\@doiabbr{hematolrep}
	\gdef\@ISSN{2038-8330}	
	\gdef\@societyowner{}
}
\DeclareOption{heritage}{%
	\gdef\@journal{heritage}
	\gdef\@journalfull{Heritage}
	\gdef\@journalshort{Heritage}
	\gdef\@doiabbr{heritage}
	\gdef\@ISSN{2571-9408}	
	\gdef\@societyowner{}
}
\DeclareOption{higheredu}{%
	\gdef\@journal{higheredu}
	\gdef\@journalfull{Trends in Higher Education}
	\gdef\@journalshort{Trends High. Educ.}
	\gdef\@doiabbr{higheredu}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{highthroughput}{%
	\gdef\@journal{highthroughput}
	\gdef\@journalfull{High-Throughput}
	\gdef\@journalshort{High-Throughput}
	\gdef\@doiabbr{ht}
	\gdef\@ISSN{2571-5135}
	\gdef\@societyowner{}
}
\DeclareOption{histories}{%
	\gdef\@journal{histories}
	\gdef\@journalfull{Histories}
	\gdef\@journalshort{Histories}
	\gdef\@doiabbr{histories}
	\gdef\@ISSN{2409-9252}	
	\gdef\@societyowner{}
}
\DeclareOption{horticulturae}{%
	\gdef\@journal{horticulturae}
	\gdef\@journalfull{Horticulturae}
	\gdef\@journalshort{Horticulturae}
	\gdef\@doiabbr{horticulturae}
	\gdef\@ISSN{2311-7524}
	\gdef\@societyowner{}
}
\DeclareOption{hospitals}{%
	\gdef\@journal{hospitals}
	\gdef\@journalfull{Hospitals}
	\gdef\@journalshort{Hospitals}
	\gdef\@doiabbr{hospitals}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{humanities}{%
	\gdef\@journal{humanities}
	\gdef\@journalfull{Humanities}
	\gdef\@journalshort{Humanities}
	\gdef\@doiabbr{h}
	\gdef\@ISSN{2076-0787}
	\gdef\@societyowner{}
}
\DeclareOption{humans}{%
	\gdef\@journal{humans}
	\gdef\@journalfull{Humans}
	\gdef\@journalshort{Humans}
	\gdef\@doiabbr{humans}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{hydrobiology}{%
	\gdef\@journal{hydrobiology}
	\gdef\@journalfull{Hydrobiology}
	\gdef\@journalshort{Hydrobiology}
	\gdef\@doiabbr{hydrobiology}
	\gdef\@ISSN{2673-9917}	
	\gdef\@societyowner{}
}
\DeclareOption{hydrogen}{%
	\gdef\@journal{hydrogen}
	\gdef\@journalfull{Hydrogen}
	\gdef\@journalshort{Hydrogen}
	\gdef\@doiabbr{hydrogen}
	\gdef\@ISSN{2673-4141}	
	\gdef\@societyowner{}
}
\DeclareOption{hydrology}{%
	\gdef\@journal{hydrology}
	\gdef\@journalfull{Hydrology}
	\gdef\@journalshort{Hydrology}
	\gdef\@doiabbr{hydrology}
	\gdef\@ISSN{2306-5338}
	\gdef\@societyowner{}
}
\DeclareOption{hygiene}{%
	\gdef\@journal{hygiene}
	\gdef\@journalfull{Hygiene}
	\gdef\@journalshort{Hygiene}
	\gdef\@doiabbr{hygiene}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{idr}{%
	\gdef\@journal{idr}
	\gdef\@journalfull{Infectious Disease Reports}
	\gdef\@journalshort{Infect. Dis. Rep.}
	\gdef\@doiabbr{idr}
	\gdef\@ISSN{2036-7449}	
	\gdef\@societyowner{}
}
\DeclareOption{iic}{%
	\gdef\@journal{iic}
	\gdef\@journalfull{Intelligent Infrastructure and Construction}
	\gdef\@journalshort{Intell. Infrastruct. Constr.}
	\gdef\@doiabbr{iic}
	\gdef\@ISSN{3042-4720}	
	\gdef\@societyowner{}
}
\DeclareOption{ijerph}{%
	\gdef\@journal{ijerph}
	\gdef\@journalfull{International Journal of Environmental Research and Public Health}
	\gdef\@journalshort{Int. J. Environ. Res. Public Health}
	\gdef\@doiabbr{ijerph}
	\gdef\@ISSN{1660-4601}
	\gdef\@societyowner{}
}
\DeclareOption{ijfs}{%
	\gdef\@journal{ijfs}
	\gdef\@journalfull{International Journal of Financial Studies}
	\gdef\@journalshort{Int. J. Financial Stud.}
	\gdef\@doiabbr{ijfs}
	\gdef\@ISSN{2227-7072}
	\gdef\@societyowner{}
}
\DeclareOption{ijgi}{%
	\gdef\@journal{ijgi}
	\gdef\@journalfull{ISPRS International Journal of Geo-Information}
	\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}
	\gdef\@doiabbr{ijgi}
	\gdef\@ISSN{2220-9964}
	\gdef\@societyowner{International Society for Photogrammetry and Remote Sensing}
}
\DeclareOption{ijmd}{%
	\gdef\@journal{ijmd}
	\gdef\@journalfull{International Journal of Medical Devices}
	\gdef\@journalshort{Int. J. Med. Devices}
	\gdef\@doiabbr{ijmd}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{ijms}{%
	\gdef\@journal{ijms}
	\gdef\@journalfull{International Journal of Molecular Sciences}
	\gdef\@journalshort{Int. J. Mol. Sci.}
	\gdef\@doiabbr{ijms}
	\gdef\@ISSN{1422-0067}
	\gdef\@societyowner{}
}
\DeclareOption{ijns}{%
	\gdef\@journal{ijns}
	\gdef\@journalfull{International Journal of Neonatal Screening}
	\gdef\@journalshort{Int. J. Neonatal Screen.}
	\gdef\@doiabbr{ijns}
	\gdef\@ISSN{2409-515X}
	\gdef\@societyowner{International Society for Neonatal Screening}
}
\DeclareOption{ijpb}{%
	\gdef\@journal{ijpb}
	\gdef\@journalfull{International Journal of Plant Biology}
	\gdef\@journalshort{Int. J. Plant Biol.}
	\gdef\@doiabbr{ijpb}
	\gdef\@ISSN{2037-0164}	
	\gdef\@societyowner{}
}
\DeclareOption{ijt}{%
	\gdef\@journal{ijt}
	\gdef\@journalfull{International Journal of Topology}
	\gdef\@journalshort{Int. J. Topol.}
	\gdef\@doiabbr{ijt}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{ijtm}{%
	\gdef\@journal{ijtm}
	\gdef\@journalfull{International Journal of Translational Medicine}
	\gdef\@journalshort{Int. J. Transl. Med.}
	\gdef\@doiabbr{ijtm}
	\gdef\@ISSN{2673-8937}	
	\gdef\@societyowner{}
}
\DeclareOption{ijtpp}{%
	\gdef\@journal{ijtpp}
	\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}
	\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}
	\gdef\@doiabbr{ijtpp}
	\gdef\@ISSN{2504-186X}
	\gdef\@societyowner{EUROTURBO}
}
\DeclareOption{ime}{%
	\gdef\@journal{ime}
	\gdef\@journalfull{International Medical Education}
	\gdef\@journalshort{Int. Med. Educ.}
	\gdef\@doiabbr{ime}
	\gdef\@ISSN{2813-141X}	
	\gdef\@societyowner{Academic Society for International Medical Education}
}
\DeclareOption{immuno}{%
	\gdef\@journal{immuno}
	\gdef\@journalfull{Immuno}
	\gdef\@journalshort{Immuno}
	\gdef\@doiabbr{immuno}
	\gdef\@ISSN{2673-5601}	
	\gdef\@societyowner{}
}
\DeclareOption{informatics}{%
	\gdef\@journal{informatics}
	\gdef\@journalfull{Informatics}
	\gdef\@journalshort{Informatics}
	\gdef\@doiabbr{informatics}
	\gdef\@ISSN{2227-9709}
	\gdef\@societyowner{}
}
\DeclareOption{information}{%
	\gdef\@journal{information}
	\gdef\@journalfull{Information}
	\gdef\@journalshort{Information}
	\gdef\@doiabbr{info}
	\gdef\@ISSN{2078-2489}
	\gdef\@societyowner{}
}
\DeclareOption{infrastructures}{%
	\gdef\@journal{infrastructures}
	\gdef\@journalfull{Infrastructures}
	\gdef\@journalshort{Infrastructures}
	\gdef\@doiabbr{infrastructures}
	\gdef\@ISSN{2412-3811}
	\gdef\@societyowner{}
}
\DeclareOption{inorganics}{%
	\gdef\@journal{inorganics}
	\gdef\@journalfull{Inorganics}
	\gdef\@journalshort{Inorganics}
	\gdef\@doiabbr{inorganics}
	\gdef\@ISSN{2304-6740}
	\gdef\@societyowner{}
}
\DeclareOption{insects}{%
	\gdef\@journal{insects}
	\gdef\@journalfull{Insects}
	\gdef\@journalshort{Insects}
	\gdef\@doiabbr{insects}
	\gdef\@ISSN{2075-4450}
	\gdef\@societyowner{}
}
\DeclareOption{instruments}{%
	\gdef\@journal{instruments}
	\gdef\@journalfull{Instruments}
	\gdef\@journalshort{Instruments}
	\gdef\@doiabbr{instruments}
	\gdef\@ISSN{2410-390X}
	\gdef\@societyowner{}
}
\DeclareOption{inventions}{%
	\gdef\@journal{inventions}
	\gdef\@journalfull{Inventions}
	\gdef\@journalshort{Inventions}
	\gdef\@doiabbr{inventions}
	\gdef\@ISSN{2411-5134}
	\gdef\@societyowner{}
}
\DeclareOption{iot}{%
	\gdef\@journal{iot}
	\gdef\@journalfull{IoT}
	\gdef\@journalshort{IoT}
	\gdef\@doiabbr{iot}
	\gdef\@ISSN{2624-831X}	
	\gdef\@societyowner{}
}
\DeclareOption{j}{%
	\gdef\@journal{j}
	\gdef\@journalfull{J}
	\gdef\@journalshort{J}
	\gdef\@doiabbr{j}
	\gdef\@ISSN{2571-8800}	
	\gdef\@societyowner{}
}
\DeclareOption{jal}{%
	\gdef\@journal{jal}
	\gdef\@journalfull{Journal of Ageing and Longevity}
	\gdef\@journalshort{J. Ageing Longev.}
	\gdef\@doiabbr{jal}
	\gdef\@ISSN{2673-9259}	
	\gdef\@societyowner{}
}
\DeclareOption{jcdd}{%
	\gdef\@journal{jcdd}
	\gdef\@journalfull{Journal of Cardiovascular Development and Disease}
	\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}
	\gdef\@doiabbr{jcdd}
	\gdef\@ISSN{2308-3425}
	\gdef\@societyowner{}
}
\DeclareOption{jcm}{%
	\gdef\@journal{jcm}
	\gdef\@journalfull{Journal of Clinical Medicine}
	\gdef\@journalshort{J. Clin. Med.}
	\gdef\@doiabbr{jcm}
	\gdef\@ISSN{2077-0383}
	\gdef\@societyowner{}
}
\DeclareOption{jcp}{%
	\gdef\@journal{jcp}
	\gdef\@journalfull{Journal of Cybersecurity and Privacy}
	\gdef\@journalshort{J. Cybersecur. Priv.}
	\gdef\@doiabbr{jcp}
	\gdef\@ISSN{2624-800X}	
	\gdef\@societyowner{}
}
\DeclareOption{jcs}{%
	\gdef\@journal{jcs}
	\gdef\@journalfull{Journal of Composites Science}
	\gdef\@journalshort{J. Compos. Sci.}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2504-477X}
	\gdef\@societyowner{}
}
\DeclareOption{jcto}{%
	\gdef\@journal{jcto}
	\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}
	\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}
	\gdef\@doiabbr{jcto}
	\gdef\@ISSN{2813-1053}	
	\gdef\@societyowner{}
}
\DeclareOption{jdad}{%
	\gdef\@journal{jdad}
	\gdef\@journalfull{Journal of Dementia and Alzheimer’s Disease}
	\gdef\@journalshort{J. Dement. Alzheimer's Dis.}
	\gdef\@doiabbr{jdad}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{jdb}{%
	\gdef\@journal{jdb}
	\gdef\@journalfull{Journal of Developmental Biology}
	\gdef\@journalshort{J. Dev. Biol.}
	\gdef\@doiabbr{jdb}
	\gdef\@ISSN{2221-3759}
	\gdef\@societyowner{}
}
\DeclareOption{jeta}{%
	\gdef\@journal{jeta}
	\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}
	\gdef\@journalshort{J. Exp. Theor. Anal.}
	\gdef\@doiabbr{jeta}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{jfb}{%
	\gdef\@journal{jfb}
	\gdef\@journalfull{Journal of Functional Biomaterials}
	\gdef\@journalshort{J. Funct. Biomater.}
	\gdef\@doiabbr{jfb}
	\gdef\@ISSN{2079-4983}
	\gdef\@societyowner{}
}
\DeclareOption{jfmk}{%
	\gdef\@journal{jfmk}
	\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}
	\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}
	\gdef\@doiabbr{jfmk}
	\gdef\@ISSN{2411-5142}
	\gdef\@societyowner{}
}
\DeclareOption{jimaging}{%
	\gdef\@journal{jimaging}
	\gdef\@journalfull{Journal of Imaging}
	\gdef\@journalshort{J. Imaging}
	\gdef\@doiabbr{jimaging}
	\gdef\@ISSN{2313-433X}
	\gdef\@societyowner{}
}
\DeclareOption{jintelligence}{%
	\gdef\@journal{jintelligence}
	\gdef\@journalfull{Journal of Intelligence}
	\gdef\@journalshort{J. Intell.}
	\gdef\@doiabbr{jintelligence}
	\gdef\@ISSN{2079-3200}
	\gdef\@societyowner{}
}
\DeclareOption{jlpea}{%
	\gdef\@journal{jlpea}
	\gdef\@journalfull{Journal of Low Power Electronics and Applications}
	\gdef\@journalshort{J. Low Power Electron. Appl.}
	\gdef\@doiabbr{jlpea}
	\gdef\@ISSN{2079-9268}
	\gdef\@societyowner{}
}
\DeclareOption{jmahp}{%
	\gdef\@journal{jmahp}
	\gdef\@journalfull{Journal of Market Access \& Health Policy}
	\gdef\@journalshort{J. Mark. Access Health Policy}
	\gdef\@doiabbr{jmahp}
	\gdef\@ISSN{2001-6689}	
	\gdef\@societyowner{Market Access Society}
}
\DeclareOption{jmmp}{%
	\gdef\@journal{jmmp}
	\gdef\@journalfull{Journal of Manufacturing and Materials Processing}
	\gdef\@journalshort{J. Manuf. Mater. Process.}
	\gdef\@doiabbr{jmmp}
	\gdef\@ISSN{2504-4494}
	\gdef\@societyowner{}
}
\DeclareOption{jmms}{%
        \gdef\@journal{jmms}
        \gdef\@journalfull{Journal of Mind and Medical Sciences}
        \gdef\@journalshort{J. Mind Med. Sci.}
        \gdef\@doiabbr{jmms}
        \gdef\@ISSN{2392-7674}
        \gdef\@societyowner{}
}
\DeclareOption{jmp}{%
	\gdef\@journal{jmp}
	\gdef\@journalfull{Journal of Molecular Pathology}
	\gdef\@journalshort{J. Mol. Pathol.}
	\gdef\@doiabbr{jmp}
	\gdef\@ISSN{2673-5261}	
	\gdef\@societyowner{}
}
\DeclareOption{jmse}{%
	\gdef\@journal{jmse}
	\gdef\@journalfull{Journal of Marine Science and Engineering}
	\gdef\@journalshort{J. Mar. Sci. Eng.}
	\gdef\@doiabbr{jmse}
	\gdef\@ISSN{2077-1312}
	\gdef\@societyowner{}
}
\DeclareOption{jne}{%
	\gdef\@journal{jne}
	\gdef\@journalfull{Journal of Nuclear Engineering}
	\gdef\@journalshort{J. Nucl. Eng.}
	\gdef\@doiabbr{jne}
	\gdef\@ISSN{2673-4362}	
	\gdef\@societyowner{}
}
\DeclareOption{jnt}{%
	\gdef\@journal{jnt}
	\gdef\@journalfull{Journal of Nanotheranostics}
	\gdef\@journalshort{J. Nanotheranostics}
	\gdef\@doiabbr{jnt}
	\gdef\@ISSN{2624-845X}	
	\gdef\@societyowner{}
} 
\DeclareOption{jof}{%
	\gdef\@journal{jof}
	\gdef\@journalfull{Journal of Fungi}
	\gdef\@journalshort{J. Fungi}
	\gdef\@doiabbr{jof}
	\gdef\@ISSN{2309-608X}
	\gdef\@societyowner{}
}
\DeclareOption{joitmc}{%
	\gdef\@journal{joitmc}
	\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}
	\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}
	\gdef\@doiabbr{joitmc}
	\gdef\@ISSN{2199-8531}
	\gdef\@societyowner{}
}
\DeclareOption{joma}{%
	\gdef\@journal{joma}
	\gdef\@journalfull{Journal of the Oman Medical Association}
	\gdef\@journalshort{J. Oman Med. Assoc.}
	\gdef\@doiabbr{joma}
	\gdef\@ISSN{2813-8759}	
	\gdef\@societyowner{Oman Medical Association}
}
\DeclareOption{jop}{%
        \gdef\@journal{jop}
        \gdef\@journalfull{Journal of Parks}
        \gdef\@journalshort{J. Parks}
       \gdef\@doiabbr{jop}
       \gdef\@ISSN{}
       \gdef\@societyowner{}
}
\DeclareOption{jor}{%
	\gdef\@journal{jor}
	\gdef\@journalfull{Journal of Respiration}
	\gdef\@journalshort{J. Respir.}
	\gdef\@doiabbr{jor}
	\gdef\@ISSN{2673-527X}	
	\gdef\@societyowner{}
}
\DeclareOption{journalmedia}{%
	\gdef\@journal{journalmedia}
	\gdef\@journalfull{Journalism and Media}
	\gdef\@journalshort{Journal. Media}
	\gdef\@doiabbr{journalmedia}
	\gdef\@ISSN{2673-5172}	
	\gdef\@societyowner{}
}
\DeclareOption{jox}{%
	\gdef\@journal{jox}
	\gdef\@journalfull{Journal of Xenobiotics}
	\gdef\@journalshort{J. Xenobiot.}
	\gdef\@doiabbr{jox}
	\gdef\@ISSN{2039-4713}	
	\gdef\@societyowner{}
}
\DeclareOption{jpbi}{%
	\gdef\@journal{jpbi}
	\gdef\@journalfull{Journal of Pharmaceutical and BioTech Industry}
	\gdef\@journalshort{J. Pharm. BioTech Ind.}
	\gdef\@doiabbr{jpbi}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{jpm}{%
	\gdef\@journal{jpm}
	\gdef\@journalfull{Journal of Personalized Medicine}
	\gdef\@journalshort{J. Pers. Med.}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{2075-4426}
	\gdef\@societyowner{}
}
\DeclareOption{jrfm}{%
	\gdef\@journal{jrfm}
	\gdef\@journalfull{Journal of Risk and Financial Management}
	\gdef\@journalshort{J. Risk Financial Manag.}
	\gdef\@doiabbr{jrfm}
	\gdef\@ISSN{1911-8074}
	\gdef\@societyowner{}
}
\DeclareOption{jsan}{%
	\gdef\@journal{jsan}
	\gdef\@journalfull{Journal of Sensor and Actuator Networks}
	\gdef\@journalshort{J. Sens. Actuator Netw.}
	\gdef\@doiabbr{jsan}
	\gdef\@ISSN{2224-2708}
	\gdef\@societyowner{}
}
\DeclareOption{jtaer}{%
	\gdef\@journal{jtaer}
	\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}
	\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}
	\gdef\@doiabbr{jtaer}
	\gdef\@ISSN{0718-1876}	
	\gdef\@societyowner{}
}
\DeclareOption{jvd}{%
	\gdef\@journal{jvd}
	\gdef\@journalfull{Journal of Vascular Diseases}
	\gdef\@journalshort{J. Vasc. Dis.}
	\gdef\@doiabbr{jvd}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{jzbg}{%
	\gdef\@journal{jzbg}
	\gdef\@journalfull{Journal of Zoological and Botanical Gardens}
	\gdef\@journalshort{J. Zool. Bot. Gard.}
	\gdef\@doiabbr{jzbg}
	\gdef\@ISSN{2673-5636}	
	\gdef\@societyowner{}
}
\DeclareOption{kidneydial}{%
	\gdef\@journal{kidneydial}
	\gdef\@journalfull{Kidney and Dialysis}
	\gdef\@journalshort{Kidney Dial.}
	\gdef\@doiabbr{kidneydial}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{kinasesphosphatases}{%
	\gdef\@journal{kinasesphosphatases}
	\gdef\@journalfull{Kinases and Phosphatases}
	\gdef\@journalshort{Kinases Phosphatases}
	\gdef\@doiabbr{kinasesphosphatases}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{knowledge}{%
	\gdef\@journal{knowledge}
	\gdef\@journalfull{Knowledge}
	\gdef\@journalshort{Knowledge}
	\gdef\@doiabbr{knowledge}
	\gdef\@ISSN{2673-9585}	
	\gdef\@societyowner{}
}
\DeclareOption{labmed}{%
	\gdef\@journal{labmed}
	\gdef\@journalfull{LabMed}
	\gdef\@journalshort{LabMed}
	\gdef\@doiabbr{labmed}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{laboratories}{%
	\gdef\@journal{laboratories}
	\gdef\@journalfull{Laboratories}
	\gdef\@journalshort{Laboratories}
	\gdef\@doiabbr{laboratories}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{land}{%
	\gdef\@journal{land}
	\gdef\@journalfull{Land}
	\gdef\@journalshort{Land}
	\gdef\@doiabbr{land}
	\gdef\@ISSN{2073-445X}
	\gdef\@societyowner{}
}
\DeclareOption{languages}{%
	\gdef\@journal{languages}
	\gdef\@journalfull{Languages}
	\gdef\@journalshort{Languages}
	\gdef\@doiabbr{languages}
	\gdef\@ISSN{2226-471X}
	\gdef\@societyowner{}
}
\DeclareOption{laws}{%
	\gdef\@journal{laws}
	\gdef\@journalfull{Laws}
	\gdef\@journalshort{Laws}
	\gdef\@doiabbr{laws}
	\gdef\@ISSN{2075-471X}
	\gdef\@societyowner{}
}
\DeclareOption{life}{%
	\gdef\@journal{life}
	\gdef\@journalfull{Life}
	\gdef\@journalshort{Life}
	\gdef\@doiabbr{life}
	\gdef\@ISSN{2075-1729}
	\gdef\@societyowner{}
}
\DeclareOption{lights}{%
	\gdef\@journal{lights}
	\gdef\@journalfull{Lights}
	\gdef\@journalshort{Lights}
	\gdef\@doiabbr{lights}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{limnolrev}{%
	\gdef\@journal{limnolrev}
	\gdef\@journalfull{Limnological Review}
	\gdef\@journalshort{Limnol. Rev.}
	\gdef\@doiabbr{limnolrev}
	\gdef\@ISSN{2300-7575}	
	\gdef\@societyowner{}
}
\DeclareOption{lipidology}{%
	\gdef\@journal{lipidology}
	\gdef\@journalfull{Lipidology}
	\gdef\@journalshort{Lipidology}
	\gdef\@doiabbr{lipidology}
	\gdef\@ISSN{2813-7086}	
	\gdef\@societyowner{}
}
\DeclareOption{liquids}{%
	\gdef\@journal{liquids}
	\gdef\@journalfull{Liquids}
	\gdef\@journalshort{Liquids}
	\gdef\@doiabbr{liquids}
	\gdef\@ISSN{2673-8015}	
	\gdef\@societyowner{}
}
\DeclareOption{literature}{%
	\gdef\@journal{literature}
	\gdef\@journalfull{Literature}
	\gdef\@journalshort{Literature}
	\gdef\@doiabbr{literature}
	\gdef\@ISSN{2410-9789}	
	\gdef\@societyowner{}
}
\DeclareOption{livers}{%
	\gdef\@journal{livers}
	\gdef\@journalfull{Livers}
	\gdef\@journalshort{Livers}
	\gdef\@doiabbr{livers}
	\gdef\@ISSN{2673-4389}	
	\gdef\@societyowner{}
}
\DeclareOption{logics}{%
	\gdef\@journal{logics}
	\gdef\@journalfull{Logics}
	\gdef\@journalshort{Logics}
	\gdef\@doiabbr{logics}
	\gdef\@ISSN{2813-0405}	
	\gdef\@societyowner{}
}
\DeclareOption{logistics}{%
	\gdef\@journal{logistics}
	\gdef\@journalfull{Logistics}
	\gdef\@journalshort{Logistics}
	\gdef\@doiabbr{logistics}
	\gdef\@ISSN{2305-6290}
	\gdef\@societyowner{}
}
\DeclareOption{lubricants}{%
	\gdef\@journal{lubricants}
	\gdef\@journalfull{Lubricants}
	\gdef\@journalshort{Lubricants}
	\gdef\@doiabbr{lubricants}
	\gdef\@ISSN{2075-4442}
	\gdef\@societyowner{}
}
\DeclareOption{lymphatics}{%
	\gdef\@journal{lymphatics}
	\gdef\@journalfull{Lymphatics}
	\gdef\@journalshort{Lymphatics}
	\gdef\@doiabbr{lymphatics}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{machines}{%
	\gdef\@journal{machines}
	\gdef\@journalfull{Machines}
	\gdef\@journalshort{Machines}
	\gdef\@doiabbr{machines}
	\gdef\@ISSN{2075-1702}
	\gdef\@societyowner{}
}
\DeclareOption{macromol}{%
	\gdef\@journal{macromol}
	\gdef\@journalfull{Macromol}
	\gdef\@journalshort{Macromol}
	\gdef\@doiabbr{macromol}
	\gdef\@ISSN{2673-6209}	
	\gdef\@societyowner{}
}
\DeclareOption{magnetism}{%
	\gdef\@journal{magnetism}
	\gdef\@journalfull{Magnetism}
	\gdef\@journalshort{Magnetism}
	\gdef\@doiabbr{magnetism}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{magnetochemistry}{%
	\gdef\@journal{magnetochemistry}
	\gdef\@journalfull{Magnetochemistry}
	\gdef\@journalshort{Magnetochemistry}
	\gdef\@doiabbr{magnetochemistry}
	\gdef\@ISSN{2312-7481}
	\gdef\@societyowner{}
}
\DeclareOption{make}{%
	\gdef\@journal{make}
	\gdef\@journalfull{Machine Learning and Knowledge Extraction}
	\gdef\@journalshort{Mach. Learn. Knowl. Extr.}
	\gdef\@doiabbr{make}
	\gdef\@ISSN{2504-4990}	
	\gdef\@societyowner{}
}
\DeclareOption{marinedrugs}{%
	\gdef\@journal{marinedrugs}
	\gdef\@journalfull{Marine Drugs}
	\gdef\@journalshort{Mar. Drugs}
	\gdef\@doiabbr{md}
	\gdef\@ISSN{1660-3397}
	\gdef\@societyowner{}
}
\DeclareOption{materials}{%
	\gdef\@journal{materials}
	\gdef\@journalfull{Materials}
	\gdef\@journalshort{Materials}
	\gdef\@doiabbr{ma}
	\gdef\@ISSN{1996-1944}
	\gdef\@societyowner{}
}
\DeclareOption{materproc}{%
	\gdef\@journal{materproc}
	\gdef\@journalfull{Materials Proceedings}
	\gdef\@journalshort{Mater. Proc.}
	\gdef\@doiabbr{materproc}
	\gdef\@ISSN{2673-4605}
	\gdef\@societyowner{}
}
\DeclareOption{mathematics}{%
	\gdef\@journal{mathematics}
	\gdef\@journalfull{Mathematics}
	\gdef\@journalshort{Mathematics}
	\gdef\@doiabbr{math}
	\gdef\@ISSN{2227-7390}
	\gdef\@societyowner{}
}
\DeclareOption{mca}{%
	\gdef\@journal{mca}
	\gdef\@journalfull{Mathematical and Computational Applications}
	\gdef\@journalshort{Math. Comput. Appl.}
	\gdef\@doiabbr{mca}
	\gdef\@ISSN{2297-8747}
	\gdef\@societyowner{}
}
\DeclareOption{measurements}{%
	\gdef\@journal{measurements}
	\gdef\@journalfull{Measurements}
	\gdef\@journalshort{Measurements}
	\gdef\@doiabbr{measurements}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{medicina}{%
	\gdef\@journal{medicina}
	\gdef\@journalfull{Medicina}
	\gdef\@journalshort{Medicina}
	\gdef\@doiabbr{medicina}
	\gdef\@ISSN{1648-9144}
	\gdef\@societyowner{Lithuanian University of Health Sciences}
}
\DeclareOption{medicines}{%
	\gdef\@journal{medicines}
	\gdef\@journalfull{Medicines}
	\gdef\@journalshort{Medicines}
	\gdef\@doiabbr{medicines}
	\gdef\@ISSN{2305-6320}
	\gdef\@societyowner{}
}
\DeclareOption{medsci}{%
	\gdef\@journal{medsci}
	\gdef\@journalfull{Medical Sciences}
	\gdef\@journalshort{Med. Sci.}
	\gdef\@doiabbr{medsci}
	\gdef\@ISSN{2076-3271}
	\gdef\@societyowner{}
}
\DeclareOption{membranes}{%
	\gdef\@journal{membranes}
	\gdef\@journalfull{Membranes}
	\gdef\@journalshort{Membranes}
	\gdef\@doiabbr{membranes}
	\gdef\@ISSN{2077-0375}
	\gdef\@societyowner{}
}
\DeclareOption{merits}{%
	\gdef\@journal{merits}
	\gdef\@journalfull{Merits}
	\gdef\@journalshort{Merits}
	\gdef\@doiabbr{merits}
	\gdef\@ISSN{2673-8104}	
	\gdef\@societyowner{}
}
\DeclareOption{metabolites}{%
	\gdef\@journal{metabolites}
	\gdef\@journalfull{Metabolites}
	\gdef\@journalshort{Metabolites}
	\gdef\@doiabbr{metabo}
	\gdef\@ISSN{2218-1989}
	\gdef\@societyowner{}
}
\DeclareOption{metals}{%
	\gdef\@journal{metals}
	\gdef\@journalfull{Metals}
	\gdef\@journalshort{Metals}
	\gdef\@doiabbr{met}
	\gdef\@ISSN{2075-4701}
	\gdef\@societyowner{}
}
\DeclareOption{meteorology}{%
	\gdef\@journal{meteorology}
	\gdef\@journalfull{Meteorology}
	\gdef\@journalshort{Meteorology}
	\gdef\@doiabbr{meteorology}
	\gdef\@ISSN{2674-0494}	
	\gdef\@societyowner{}
}
\DeclareOption{methane}{%
	\gdef\@journal{methane}
	\gdef\@journalfull{Methane}
	\gdef\@journalshort{Methane}
	\gdef\@doiabbr{methane}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{metrics}{%
	\gdef\@journal{metrics}
	\gdef\@journalfull{Metrics}
	\gdef\@journalshort{Metrics}
	\gdef\@doiabbr{metrics}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{metrology}{%
	\gdef\@journal{metrology}
	\gdef\@journalfull{Metrology}
	\gdef\@journalshort{Metrology}
	\gdef\@doiabbr{metrology}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{micro}{%
	\gdef\@journal{micro}
	\gdef\@journalfull{Micro}
	\gdef\@journalshort{Micro}
	\gdef\@doiabbr{micro}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{microarrays}{%
	\gdef\@journal{microarrays}
	\gdef\@journalfull{Microarrays}
	\gdef\@journalshort{Microarrays}
	\gdef\@doiabbr{microarrays}
	\gdef\@ISSN{2076-3905}
	\gdef\@societyowner{}
}
\DeclareOption{microbiolres}{%
	\gdef\@journal{microbiolres}
	\gdef\@journalfull{Microbiology Research}
	\gdef\@journalshort{Microbiol. Res.}
	\gdef\@doiabbr{microbiolres}
	\gdef\@ISSN{2036-7481}	
	\gdef\@societyowner{}
}
\DeclareOption{microelectronics}{%
       \gdef\@journal{microelectronics}
       \gdef\@journalfull{Microelectronics}
       \gdef\@journalshort{Microelectronics}
       \gdef\@doiabbr{microelectronics}
       \gdef\@ISSN{}       
       \gdef\@societyowner{}
}
\DeclareOption{micromachines}{%
	\gdef\@journal{micromachines}
	\gdef\@journalfull{Micromachines}
	\gdef\@journalshort{Micromachines}
	\gdef\@doiabbr{mi}
	\gdef\@ISSN{2072-666X}
	\gdef\@societyowner{}
}
\DeclareOption{microorganisms}{%
	\gdef\@journal{microorganisms}
	\gdef\@journalfull{Microorganisms}
	\gdef\@journalshort{Microorganisms}
	\gdef\@doiabbr{microorganisms}
	\gdef\@ISSN{2076-2607}
	\gdef\@societyowner{}
}
\DeclareOption{microplastics}{%
	\gdef\@journal{microplastics}
	\gdef\@journalfull{Microplastics}
	\gdef\@journalshort{Microplastics}
	\gdef\@doiabbr{microplastics}
	\gdef\@ISSN{2673-8929}	
	\gdef\@societyowner{}
}
\DeclareOption{microwave}{%
	\gdef\@journal{microwave}
	\gdef\@journalfull{Microwave}
	\gdef\@journalshort{Microwave}
	\gdef\@doiabbr{microwave}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{minerals}{%
	\gdef\@journal{minerals}
	\gdef\@journalfull{Minerals}
	\gdef\@journalshort{Minerals}
	\gdef\@doiabbr{min}
	\gdef\@ISSN{2075-163X}
	\gdef\@societyowner{}
}
\DeclareOption{mining}{%
	\gdef\@journal{mining}
	\gdef\@journalfull{Mining}
	\gdef\@journalshort{Mining}
	\gdef\@doiabbr{mining}
	\gdef\@ISSN{2673-6489}	
	\gdef\@societyowner{}
}
\DeclareOption{mmphys}{%
        \gdef\@journal{mmphys}
        \gdef\@journalfull{Modern Mathematical Physics}
        \gdef\@journalshort{Mod. Math. Phys.}
        \gdef\@doiabbr{mmphys}
        \gdef\@ISSN{3042-5034}        
       \gdef\@societyowner{}
}
\DeclareOption{modelling}{%
	\gdef\@journal{modelling}
	\gdef\@journalfull{Modelling}
	\gdef\@journalshort{Modelling}
	\gdef\@doiabbr{modelling}
	\gdef\@ISSN{2673-3951}	
	\gdef\@societyowner{}
}
\DeclareOption{molbank}{%
	\gdef\@journal{molbank}
	\gdef\@journalfull{Molbank}
	\gdef\@journalshort{Molbank}
	\gdef\@doiabbr{M}
	\gdef\@ISSN{1422-8599}
	\gdef\@societyowner{}
}
\DeclareOption{molecules}{%
	\gdef\@journal{molecules}
	\gdef\@journalfull{Molecules}
	\gdef\@journalshort{Molecules}
	\gdef\@doiabbr{molecules}
	\gdef\@ISSN{1420-3049}
	\gdef\@societyowner{}
}
\DeclareOption{mps}{%
	\gdef\@journal{mps}
	\gdef\@journalfull{Methods and Protocols}
	\gdef\@journalshort{Methods Protoc.}
	\gdef\@doiabbr{mps}
	\gdef\@ISSN{2409-9279}
	\gdef\@societyowner{}
}
\DeclareOption{msf}{%
	\gdef\@journal{msf}
	\gdef\@journalfull{Medical Sciences Forum}
	\gdef\@journalshort{Med. Sci. Forum}
	\gdef\@doiabbr{msf}
	\gdef\@ISSN{2673-9992}
	\gdef\@societyowner{}
}
\DeclareOption{mti}{%
	\gdef\@journal{mti}
	\gdef\@journalfull{Multimodal Technologies and Interaction}
	\gdef\@journalshort{Multimodal Technol. Interact.}
	\gdef\@doiabbr{mti}
	\gdef\@ISSN{2414-4088}
	\gdef\@societyowner{}
}
\DeclareOption{multimedia}{%
       \gdef\@journal{multimedia}
       \gdef\@journalfull{Multimedia}
       \gdef\@journalshort{Multimedia}
       \gdef\@doiabbr{multimedia}
       \gdef\@ISSN{}       
       \gdef\@societyowner{}
}
\DeclareOption{muscles}{%
	\gdef\@journal{muscles}
	\gdef\@journalfull{Muscles}
	\gdef\@journalshort{Muscles}
	\gdef\@doiabbr{muscles}
	\gdef\@ISSN{2813-0413}	
	\gdef\@societyowner{}
}
\DeclareOption{nanoenergyadv}{%
	\gdef\@journal{nanoenergyadv}
	\gdef\@journalfull{Nanoenergy Advances}
	\gdef\@journalshort{Nanoenergy Adv.}
	\gdef\@doiabbr{nanoenergyadv}
	\gdef\@ISSN{2673-706X}	
	\gdef\@societyowner{}
}
\DeclareOption{nanomanufacturing}{%
	\gdef\@journal{nanomanufacturing}
	\gdef\@journalfull{Nanomanufacturing}
	\gdef\@journalshort{Nanomanufacturing}
	\gdef\@doiabbr{nanomanufacturing}
	\gdef\@ISSN{2673-687X}	
	\gdef\@societyowner{}
}
\DeclareOption{nanomaterials}{%
	\gdef\@journal{nanomaterials}
	\gdef\@journalfull{Nanomaterials}
	\gdef\@journalshort{Nanomaterials}
	\gdef\@doiabbr{nano}
	\gdef\@ISSN{2079-4991}
	\gdef\@societyowner{}
}
\DeclareOption{ncrna}{%
	\gdef\@journal{ncrna}
	\gdef\@journalfull{Non-Coding RNA}
	\gdef\@journalshort{Non-Coding RNA}
	\gdef\@doiabbr{ncrna}
	\gdef\@ISSN{2311-553X}
	\gdef\@societyowner{}
}
\DeclareOption{ndt}{%
	\gdef\@journal{ndt}
	\gdef\@journalfull{NDT}
	\gdef\@journalshort{NDT}
	\gdef\@doiabbr{ndt}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{network}{%
	\gdef\@journal{network}
	\gdef\@journalfull{Network}
	\gdef\@journalshort{Network}
	\gdef\@doiabbr{network}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{neuroglia}{%
	\gdef\@journal{neuroglia}
	\gdef\@journalfull{Neuroglia}
	\gdef\@journalshort{Neuroglia}
	\gdef\@doiabbr{neuroglia}
	\gdef\@ISSN{2571-6980}	
	\gdef\@societyowner{}
}
\DeclareOption{neurolint}{%
	\gdef\@journal{neurolint}
	\gdef\@journalfull{Neurology International}
	\gdef\@journalshort{Neurol. Int.}
	\gdef\@doiabbr{neurolint}
	\gdef\@ISSN{2035-8377}	
	\gdef\@societyowner{}
}
\DeclareOption{neurosci}{%
	\gdef\@journal{neurosci}
	\gdef\@journalfull{NeuroSci}
	\gdef\@journalshort{NeuroSci}
	\gdef\@doiabbr{neurosci}
	\gdef\@ISSN{2673-4087}	
	\gdef\@societyowner{}
}
\DeclareOption{nitrogen}{%
	\gdef\@journal{nitrogen}
	\gdef\@journalfull{Nitrogen}
	\gdef\@journalshort{Nitrogen}
	\gdef\@doiabbr{nitrogen}
	\gdef\@ISSN{2504-3129}	
	\gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{nri}{%
	\gdef\@journal{nri}
	\gdef\@journalfull{Natural Resources Informatics}
	\gdef\@journalshort{Nat. Resour. Inform.}
	\gdef\@doiabbr{nri}
	\gdef\@ISSN{2673-981X}	
	\gdef\@societyowner{}
}
\DeclareOption{nursrep}{%
	\gdef\@journal{nursrep}
	\gdef\@journalfull{Nursing Reports}
	\gdef\@journalshort{Nurs. Rep.}
	\gdef\@doiabbr{nursrep}
	\gdef\@ISSN{2039-4403}	
	\gdef\@societyowner{}
}
\DeclareOption{nutraceuticals}{%
	\gdef\@journal{nutraceuticals}
	\gdef\@journalfull{Nutraceuticals}
	\gdef\@journalshort{Nutraceuticals}
	\gdef\@doiabbr{nutraceuticals}
	\gdef\@ISSN{1661-3821}	
	\gdef\@societyowner{}
}
\DeclareOption{nutrients}{%
	\gdef\@journal{nutrients}
	\gdef\@journalfull{Nutrients}
	\gdef\@journalshort{Nutrients}
	\gdef\@doiabbr{nu}
	\gdef\@ISSN{2072-6643}
	\gdef\@societyowner{}
}
\DeclareOption{obesities}{%
	\gdef\@journal{obesities}
	\gdef\@journalfull{Obesities}
	\gdef\@journalshort{Obesities}
	\gdef\@doiabbr{obesities}
	\gdef\@ISSN{2673-4168}	
	\gdef\@societyowner{}
}
\DeclareOption{oceans}{%
	\gdef\@journal{oceans}
	\gdef\@journalfull{Oceans}
	\gdef\@journalshort{Oceans}
	\gdef\@doiabbr{oceans}
	\gdef\@ISSN{2673-1924}	
	\gdef\@societyowner{}
}
\DeclareOption{ohbm}{%
	\gdef\@journal{ohbm}
	\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}
	\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}
	\gdef\@doiabbr{ohbm}
	\gdef\@ISSN{2504-463X}
	\gdef\@societyowner{}
}
\DeclareOption{onco}{%
	\gdef\@journal{onco}
	\gdef\@journalfull{Onco}
	\gdef\@journalshort{Onco}
	\gdef\@doiabbr{onco}
	\gdef\@ISSN{2673-7523}	
	\gdef\@societyowner{}
}
\DeclareOption{optics}{%
	\gdef\@journal{optics}
	\gdef\@journalfull{Optics}
	\gdef\@journalshort{Optics}
	\gdef\@doiabbr{opt}
	\gdef\@ISSN{2673-3269}	
	\gdef\@societyowner{}
}
\DeclareOption{oral}{%
	\gdef\@journal{oral}
	\gdef\@journalfull{Oral}
	\gdef\@journalshort{Oral}
	\gdef\@doiabbr{oral}
	\gdef\@ISSN{2673-6373}	
	\gdef\@societyowner{}
}
\DeclareOption{organics}{%
	\gdef\@journal{organics}
	\gdef\@journalfull{Organics}
	\gdef\@journalshort{Organics}
	\gdef\@doiabbr{org}
	\gdef\@ISSN{2673-401X}	
	\gdef\@societyowner{}
}
\DeclareOption{organoids}{%
	\gdef\@journal{organoids}
	\gdef\@journalfull{Organoids}
	\gdef\@journalshort{Organoids}
	\gdef\@doiabbr{organoids}
	\gdef\@ISSN{2674-1172}	
	\gdef\@societyowner{}
}
\DeclareOption{osteology}{%
	\gdef\@journal{osteology}
	\gdef\@journalfull{Osteology}
	\gdef\@journalshort{Osteology}
	\gdef\@doiabbr{osteology}
	\gdef\@ISSN{2673-4036}	
	\gdef\@societyowner{}
}
\DeclareOption{oxygen}{%
	\gdef\@journal{oxygen}
	\gdef\@journalfull{Oxygen}
	\gdef\@journalshort{Oxygen}
	\gdef\@doiabbr{oxygen}
	\gdef\@ISSN{2673-9801}	
	\gdef\@societyowner{}
}
\DeclareOption{parasites}{%
	\gdef\@journal{parasites}
	\gdef\@journalfull{Parasites}
	\gdef\@journalshort{Parasites}
	\gdef\@doiabbr{parasites}
	\gdef\@ISSN{2673-5946}
	\gdef\@societyowner{}
}
\DeclareOption{parasitologia}{%
	\gdef\@journal{parasitologia}
	\gdef\@journalfull{Parasitologia}
	\gdef\@journalshort{Parasitologia}
	\gdef\@doiabbr{parasitologia}
	\gdef\@ISSN{2673-6772}	
	\gdef\@societyowner{}
}
\DeclareOption{particles}{%
	\gdef\@journal{particles}
	\gdef\@journalfull{Particles}
	\gdef\@journalshort{Particles}
	\gdef\@doiabbr{particles}
	\gdef\@ISSN{2571-712X}	
	\gdef\@societyowner{}
}
\DeclareOption{pathogens}{%
	\gdef\@journal{pathogens}
	\gdef\@journalfull{Pathogens}
	\gdef\@journalshort{Pathogens}
	\gdef\@doiabbr{pathogens}
	\gdef\@ISSN{2076-0817}
	\gdef\@societyowner{}
}
\DeclareOption{pathophysiology}{%
	\gdef\@journal{pathophysiology}
	\gdef\@journalfull{Pathophysiology}
	\gdef\@journalshort{Pathophysiology}
	\gdef\@doiabbr{pathophysiology}
	\gdef\@ISSN{0928-4680}	
	\gdef\@societyowner{}
}
\DeclareOption{pediatrrep}{%
	\gdef\@journal{pediatrrep}
	\gdef\@journalfull{Pediatric Reports}
	\gdef\@journalshort{Pediatr. Rep.}
	\gdef\@doiabbr{pediatric}
	\gdef\@ISSN{2036-7503}	
	\gdef\@societyowner{}
}
\DeclareOption{pets}{%
	\gdef\@journal{pets}
	\gdef\@journalfull{Pets}
	\gdef\@journalshort{Pets}
	\gdef\@doiabbr{pets}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{pharmaceuticals}{%
	\gdef\@journal{pharmaceuticals}
	\gdef\@journalfull{Pharmaceuticals}
	\gdef\@journalshort{Pharmaceuticals}
	\gdef\@doiabbr{ph}
	\gdef\@ISSN{1424-8247}
	\gdef\@societyowner{}
}
\DeclareOption{pharmaceutics}{%
	\gdef\@journal{pharmaceutics}
	\gdef\@journalfull{Pharmaceutics}
	\gdef\@journalshort{Pharmaceutics}
	\gdef\@doiabbr{pharmaceutics}
	\gdef\@ISSN{1999-4923}
	\gdef\@societyowner{}
}
\DeclareOption{pharmacoepidemiology}{%
	\gdef\@journal{pharmacoepidemiology}
	\gdef\@journalfull{Pharmacoepidemiology}
	\gdef\@journalshort{Pharmacoepidemiology}
	\gdef\@doiabbr{pharma}
	\gdef\@ISSN{2813-0618}	
	\gdef\@societyowner{}
}
\DeclareOption{pharmacy}{%
	\gdef\@journal{pharmacy}
	\gdef\@journalfull{Pharmacy}
	\gdef\@journalshort{Pharmacy}
	\gdef\@doiabbr{pharmacy}
	\gdef\@ISSN{2226-4787}
	\gdef\@societyowner{}
}
\DeclareOption{philosophies}{%
	\gdef\@journal{philosophies}
	\gdef\@journalfull{Philosophies}
	\gdef\@journalshort{Philosophies}
	\gdef\@doiabbr{philosophies}
	\gdef\@ISSN{2409-9287}
	\gdef\@societyowner{}
}
\DeclareOption{photochem}{%
	\gdef\@journal{photochem}
	\gdef\@journalfull{Photochem}
	\gdef\@journalshort{Photochem}
	\gdef\@doiabbr{photochem}
	\gdef\@ISSN{2673-7256}	
	\gdef\@societyowner{}
}
\DeclareOption{photonics}{%
	\gdef\@journal{photonics}
	\gdef\@journalfull{Photonics}
	\gdef\@journalshort{Photonics}
	\gdef\@doiabbr{photonics}
	\gdef\@ISSN{2304-6732}
	\gdef\@societyowner{}
}
\DeclareOption{phycology}{%
	\gdef\@journal{phycology}
	\gdef\@journalfull{Phycology}
	\gdef\@journalshort{Phycology}
	\gdef\@doiabbr{phycology}
	\gdef\@ISSN{2673-9410}	
	\gdef\@societyowner{}
}
\DeclareOption{physchem}{%
	\gdef\@journal{physchem}
	\gdef\@journalfull{Physchem}
	\gdef\@journalshort{Physchem}
	\gdef\@doiabbr{physchem}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{physics}{%
	\gdef\@journal{physics}
	\gdef\@journalfull{Physics}
	\gdef\@journalshort{Physics}
	\gdef\@doiabbr{physics}
	\gdef\@ISSN{2624-8174}	
	\gdef\@societyowner{}
}
\DeclareOption{physiologia}{%
	\gdef\@journal{physiologia}
	\gdef\@journalfull{Physiologia}
	\gdef\@journalshort{Physiologia}
	\gdef\@doiabbr{physiologia}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{plants}{%
	\gdef\@journal{plants}
	\gdef\@journalfull{Plants}
	\gdef\@journalshort{Plants}
	\gdef\@doiabbr{plants}
	\gdef\@ISSN{2223-7747}
	\gdef\@societyowner{}
}
\DeclareOption{plasma}{%
	\gdef\@journal{plasma}
	\gdef\@journalfull{Plasma}
	\gdef\@journalshort{Plasma}
	\gdef\@doiabbr{plasma}
	\gdef\@ISSN{2571-6182}	
	\gdef\@societyowner{}
}
\DeclareOption{platforms}{%
	\gdef\@journal{platforms}
	\gdef\@journalfull{Platforms}
	\gdef\@journalshort{Platforms}
	\gdef\@doiabbr{platforms}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{pollutants}{%
	\gdef\@journal{pollutants}
	\gdef\@journalfull{Pollutants}
	\gdef\@journalshort{Pollutants}
	\gdef\@doiabbr{pollutants}
	\gdef\@ISSN{2673-4672}	
	\gdef\@societyowner{}
}
\DeclareOption{polymers}{%
	\gdef\@journal{polymers}
	\gdef\@journalfull{Polymers}
	\gdef\@journalshort{Polymers}
	\gdef\@doiabbr{polym}
	\gdef\@ISSN{2073-4360}
	\gdef\@societyowner{}
}
\DeclareOption{polysaccharides}{%
	\gdef\@journal{polysaccharides}
	\gdef\@journalfull{Polysaccharides}
	\gdef\@journalshort{Polysaccharides}
	\gdef\@doiabbr{polysaccharides}
	\gdef\@ISSN{2673-4176}	
	\gdef\@societyowner{}
}
\DeclareOption{populations}{%
	\gdef\@journal{populations}
	\gdef\@journalfull{Populations}
	\gdef\@journalshort{Populations}
	\gdef\@doiabbr{populations}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{poultry}{%
	\gdef\@journal{poultry}
	\gdef\@journalfull{Poultry}
	\gdef\@journalshort{Poultry}
	\gdef\@doiabbr{poultry}
	\gdef\@ISSN{2674-1164}	
	\gdef\@societyowner{}
}
\DeclareOption{powders}{%
	\gdef\@journal{powders}
	\gdef\@journalfull{Powders}
	\gdef\@journalshort{Powders}
	\gdef\@doiabbr{powders}
	\gdef\@ISSN{2674-0516}	
	\gdef\@societyowner{}
}
\DeclareOption{preprints}{%
	\gdef\@journal{preprints}
	\gdef\@journalfull{Preprints}
	\gdef\@journalshort{Preprints}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{preprintschicago}{% Used for chicago preprints
	\gdef\@journal{preprintschicago}
	\gdef\@journalfull{Preprints}
	\gdef\@journalshort{Preprints}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{preprintsapa}{% Used for APA preprints
	\gdef\@journal{preprintsapa}
	\gdef\@journalfull{Preprints}
	\gdef\@journalshort{Preprints}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{proceedings}{%
	\gdef\@journal{proceedings}
	\gdef\@journalfull{Proceedings}
	\gdef\@journalshort{Proceedings}
	\gdef\@doiabbr{proceedings}
	\gdef\@ISSN{2504-3900}
	\gdef\@societyowner{}
}
\DeclareOption{processes}{%
	\gdef\@journal{processes}
	\gdef\@journalfull{Processes}
	\gdef\@journalshort{Processes}
	\gdef\@doiabbr{pr}
	\gdef\@ISSN{2227-9717}
	\gdef\@societyowner{}
}
\DeclareOption{prosthesis}{%
	\gdef\@journal{prosthesis}
	\gdef\@journalfull{Prosthesis}
	\gdef\@journalshort{Prosthesis}
	\gdef\@doiabbr{prosthesis}
	\gdef\@ISSN{2673-1592}	
	\gdef\@societyowner{}
}
\DeclareOption{proteomes}{%
	\gdef\@journal{proteomes}
	\gdef\@journalfull{Proteomes}
	\gdef\@journalshort{Proteomes}
	\gdef\@doiabbr{proteomes}
	\gdef\@ISSN{2227-7382}
	\gdef\@societyowner{}
}
\DeclareOption{psf}{%
	\gdef\@journal{psf}
	\gdef\@journalfull{Physical Sciences Forum}
	\gdef\@journalshort{Phys. Sci. Forum}
	\gdef\@doiabbr{psf}
	\gdef\@ISSN{2673-9984}
	\gdef\@societyowner{}
}
\DeclareOption{psychiatryint}{%
	\gdef\@journal{psychiatryint}
	\gdef\@journalfull{Psychiatry International}
	\gdef\@journalshort{Psychiatry Int.}
	\gdef\@doiabbr{psychiatryint}
	\gdef\@ISSN{2673-5318}	
	\gdef\@societyowner{}
}
\DeclareOption{psychoactives}{%
	\gdef\@journal{psychoactives}
	\gdef\@journalfull{Psychoactives}
	\gdef\@journalshort{Psychoactives}
	\gdef\@doiabbr{psychoactives}
	\gdef\@ISSN{2813-1851}	
	\gdef\@societyowner{}
}
\DeclareOption{psycholint}{%
	\gdef\@journal{psycholint}
	\gdef\@journalfull{Psychology International}
	\gdef\@journalshort{Psychol. Int.}
	\gdef\@doiabbr{psycholint}
	\gdef\@ISSN{2813-9844}	
	\gdef\@societyowner{}
}
\DeclareOption{publications}{%
	\gdef\@journal{publications}
	\gdef\@journalfull{Publications}
	\gdef\@journalshort{Publications}
	\gdef\@doiabbr{publications}
	\gdef\@ISSN{2304-6775}
	\gdef\@societyowner{}
}
\DeclareOption{purification}{%
	\gdef\@journal{purification}
	\gdef\@journalfull{Purification}
	\gdef\@journalshort{Purification}
	\gdef\@doiabbr{purification}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{quantumrep}{%
	\gdef\@journal{quantumrep}
	\gdef\@journalfull{Quantum Reports}
	\gdef\@journalshort{Quantum Rep.}
	\gdef\@doiabbr{quantum}
	\gdef\@ISSN{2624-960X}	
	\gdef\@societyowner{}
}
\DeclareOption{quaternary}{%
	\gdef\@journal{quaternary}
	\gdef\@journalfull{Quaternary}
	\gdef\@journalshort{Quaternary}
	\gdef\@doiabbr{quat}
	\gdef\@ISSN{2571-550X}
	\gdef\@societyowner{}
}
\DeclareOption{qubs}{%
	\gdef\@journal{qubs}
	\gdef\@journalfull{Quantum Beam Science}
	\gdef\@journalshort{Quantum Beam Sci.}
	\gdef\@doiabbr{qubs}
	\gdef\@ISSN{2412-382X}
	\gdef\@societyowner{}
}
\DeclareOption{radiation}{%
	\gdef\@journal{radiation}
	\gdef\@journalfull{Radiation}
	\gdef\@journalshort{Radiation}
	\gdef\@doiabbr{radiation}
	\gdef\@ISSN{2673-592X}	
	\gdef\@societyowner{}
}
\DeclareOption{reactions}{%
	\gdef\@journal{reactions}
	\gdef\@journalfull{Reactions}
	\gdef\@journalshort{Reactions}
	\gdef\@doiabbr{reactions}
	\gdef\@ISSN{2624-781X}	
	\gdef\@societyowner{}
}
\DeclareOption{realestate}{%
	\gdef\@journal{realestate}
	\gdef\@journalfull{Real Estate}
	\gdef\@journalshort{Real Estate}
	\gdef\@doiabbr{realestate}
	\gdef\@ISSN{2813-8090}	
	\gdef\@societyowner{}
}
\DeclareOption{receptors}{%
	\gdef\@journal{receptors}
	\gdef\@journalfull{Receptors}
	\gdef\@journalshort{Receptors}
	\gdef\@doiabbr{receptors}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{recycling}{%
	\gdef\@journal{recycling}
	\gdef\@journalfull{Recycling}
	\gdef\@journalshort{Recycling}
	\gdef\@doiabbr{recycling}
	\gdef\@ISSN{2313-4321}
	\gdef\@societyowner{}
}
\DeclareOption{regeneration}{%
	\gdef\@journal{regeneration}
	\gdef\@journalfull{Regeneration}
	\gdef\@journalshort{Regeneration}
	\gdef\@doiabbr{regeneration}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{religions}{%
	\gdef\@journal{religions}
	\gdef\@journalfull{Religions}
	\gdef\@journalshort{Religions}
	\gdef\@doiabbr{rel}
	\gdef\@ISSN{2077-1444}
	\gdef\@societyowner{}
}
\DeclareOption{remotesensing}{%
	\gdef\@journal{remotesensing}
	\gdef\@journalfull{Remote Sensing}
	\gdef\@journalshort{Remote Sens.}
	\gdef\@doiabbr{rs}
	\gdef\@ISSN{2072-4292}
	\gdef\@societyowner{}
}
\DeclareOption{reports}{%
	\gdef\@journal{reports}
	\gdef\@journalfull{Reports}
	\gdef\@journalshort{Reports}
	\gdef\@doiabbr{reports}
	\gdef\@ISSN{2571-841X}
	\gdef\@societyowner{}
}
\DeclareOption{reprodmed}{%
	\gdef\@journal{reprodmed}
	\gdef\@journalfull{Reproductive Medicine}
	\gdef\@journalshort{Reprod. Med.}
	\gdef\@doiabbr{reprodmed}
	\gdef\@ISSN{2673-3897}	
	\gdef\@societyowner{}
}
\DeclareOption{resources}{%
	\gdef\@journal{resources}
	\gdef\@journalfull{Resources}
	\gdef\@journalshort{Resources}
	\gdef\@doiabbr{resources}
	\gdef\@ISSN{2079-9276}
	\gdef\@societyowner{}
}
\DeclareOption{rheumato}{%
	\gdef\@journal{rheumato}
	\gdef\@journalfull{Rheumato}
	\gdef\@journalshort{Rheumato}
	\gdef\@doiabbr{rheumato}
	\gdef\@ISSN{2674-0621}	
	\gdef\@societyowner{}
}
\DeclareOption{risks}{%
	\gdef\@journal{risks}
	\gdef\@journalfull{Risks}
	\gdef\@journalshort{Risks}
	\gdef\@doiabbr{risks}
	\gdef\@ISSN{2227-9091}
	\gdef\@societyowner{}
}
\DeclareOption{robotics}{%
	\gdef\@journal{robotics}
	\gdef\@journalfull{Robotics}
	\gdef\@journalshort{Robotics}
	\gdef\@doiabbr{robotics}
	\gdef\@ISSN{2218-6581}
	\gdef\@societyowner{}
}
\DeclareOption{rsee}{%
	\gdef\@journal{rsee}
	\gdef\@journalfull{Regional Science and Environmental Economics}
	\gdef\@journalshort{Reg. Sci. Environ. Econ.}
	\gdef\@doiabbr{rsee}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{ruminants}{%
	\gdef\@journal{ruminants}
	\gdef\@journalfull{Ruminants}
	\gdef\@journalshort{Ruminants}
	\gdef\@doiabbr{ruminants}
	\gdef\@ISSN{2673-933X}	
	\gdef\@societyowner{}
}
\DeclareOption{safety}{%
	\gdef\@journal{safety}
	\gdef\@journalfull{Safety}
	\gdef\@journalshort{Safety}
	\gdef\@doiabbr{safety}
	\gdef\@ISSN{2313-576X}
	\gdef\@societyowner{}
}
\DeclareOption{sci}{%
	\gdef\@journal{sci}
	\gdef\@journalfull{Sci}
	\gdef\@journalshort{Sci}
	\gdef\@doiabbr{sci}
	\gdef\@ISSN{2413-4155}
	\gdef\@societyowner{}
}
\DeclareOption{scipharm}{%
	\gdef\@journal{scipharm}
	\gdef\@journalfull{Scientia Pharmaceutica}
	\gdef\@journalshort{Sci. Pharm.}
	\gdef\@doiabbr{scipharm}
	\gdef\@ISSN{2218-0532}
	\gdef\@societyowner{\"{O}sterreichische Pharmazeutische Gesellschaft}
}
\DeclareOption{sclerosis}{%
	\gdef\@journal{sclerosis}
	\gdef\@journalfull{Sclerosis}
	\gdef\@journalshort{Sclerosis}
	\gdef\@doiabbr{sclerosis}
	\gdef\@ISSN{2813-3064}	
	\gdef\@societyowner{}
}
\DeclareOption{seeds}{%
	\gdef\@journal{seeds}
	\gdef\@journalfull{Seeds}
	\gdef\@journalshort{Seeds}
	\gdef\@doiabbr{seeds}
	\gdef\@ISSN{2674-1024}	
	\gdef\@societyowner{}
}
\DeclareOption{sensors}{%
	\gdef\@journal{sensors}
	\gdef\@journalfull{Sensors}
	\gdef\@journalshort{Sensors}
	\gdef\@doiabbr{s}
	\gdef\@ISSN{1424-8220}
	\gdef\@societyowner{}
}
\DeclareOption{separations}{%
	\gdef\@journal{separations}
	\gdef\@journalfull{Separations}
	\gdef\@journalshort{Separations}
	\gdef\@doiabbr{separations}
	\gdef\@ISSN{2297-8739}
	\gdef\@societyowner{}
}
\DeclareOption{sexes}{%
	\gdef\@journal{sexes}
	\gdef\@journalfull{Sexes}
	\gdef\@journalshort{Sexes}
	\gdef\@doiabbr{sexes}
	\gdef\@ISSN{2411-5118}	
	\gdef\@societyowner{}
}
\DeclareOption{signals}{%
	\gdef\@journal{signals}
	\gdef\@journalfull{Signals}
	\gdef\@journalshort{Signals}
	\gdef\@doiabbr{signals}
	\gdef\@ISSN{2624-6120}	
	\gdef\@societyowner{}
}
\DeclareOption{sinusitis}{%
	\gdef\@journal{sinusitis}
	\gdef\@journalfull{Sinusitis}
	\gdef\@journalshort{Sinusitis}
	\gdef\@doiabbr{sinusitis}
	\gdef\@ISSN{2309-107X}	
	\gdef\@societyowner{}
}
\DeclareOption{siuj}{%
	\gdef\@journal{siuj}
	\gdef\@journalfull{Soci\'{e}t\'{e} Internationale d'Urologie Journal}
	\gdef\@journalshort{Soc. Int. Urol. J.}
	\gdef\@doiabbr{siuj}
	\gdef\@ISSN{2563-6499}	
	\gdef\@societyowner{Soci\'{e}t\'{e} Internationale d'Urologie}
}
\DeclareOption{skins}{%
	\gdef\@journal{skins}
	\gdef\@journalfull{Skins}
	\gdef\@journalshort{Skins}
	\gdef\@doiabbr{skins}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{smartcities}{%
	\gdef\@journal{smartcities}
	\gdef\@journalfull{Smart Cities}
	\gdef\@journalshort{Smart Cities}
	\gdef\@doiabbr{smartcities}
	\gdef\@ISSN{2624-6511}	
	\gdef\@societyowner{}
}
\DeclareOption{sna}{%
	\gdef\@journal{sna}
	\gdef\@journalfull{Sinusitis and Asthma}
	\gdef\@journalshort{Sinusitis Asthma}
	\gdef\@doiabbr{sna}
	\gdef\@ISSN{2624-7003}
	\gdef\@societyowner{}
}
\DeclareOption{societies}{%
	\gdef\@journal{societies}
	\gdef\@journalfull{Societies}
	\gdef\@journalshort{Societies}
	\gdef\@doiabbr{soc}
	\gdef\@ISSN{2075-4698}
	\gdef\@societyowner{}
}
\DeclareOption{socsci}{%
	\gdef\@journal{socsci}
	\gdef\@journalfull{Social Sciences}
	\gdef\@journalshort{Soc. Sci.}
	\gdef\@doiabbr{socsci}
	\gdef\@ISSN{2076-0760}
	\gdef\@societyowner{}
}
\DeclareOption{software}{%
	\gdef\@journal{software}
	\gdef\@journalfull{Software}
	\gdef\@journalshort{Software}
	\gdef\@doiabbr{software}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{soilsystems}{%
	\gdef\@journal{soilsystems}
	\gdef\@journalfull{Soil Systems}
	\gdef\@journalshort{Soil Syst.}
	\gdef\@doiabbr{soilsystems}
	\gdef\@ISSN{2571-8789}
	\gdef\@societyowner{}
}
\DeclareOption{solar}{%
	\gdef\@journal{solar}
	\gdef\@journalfull{Solar}
	\gdef\@journalshort{Solar}
	\gdef\@doiabbr{solar}
	\gdef\@ISSN{2673-9941}	
	\gdef\@societyowner{}
}
\DeclareOption{solids}{%
	\gdef\@journal{solids}
	\gdef\@journalfull{Solids}
	\gdef\@journalshort{Solids}
	\gdef\@doiabbr{solids}
	\gdef\@ISSN{2673-6497}	
	\gdef\@societyowner{}
}
\DeclareOption{spectroscj}{%
	\gdef\@journal{spectroscj}
	\gdef\@journalfull{Spectroscopy Journal}
	\gdef\@journalshort{Spectrosc. J.}
	\gdef\@doiabbr{spectroscj}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{sports}{%
	\gdef\@journal{sports}
	\gdef\@journalfull{Sports}
	\gdef\@journalshort{Sports}
	\gdef\@doiabbr{sports}
	\gdef\@ISSN{2075-4663}
	\gdef\@societyowner{}
}
\DeclareOption{standards}{%
	\gdef\@journal{standards}
	\gdef\@journalfull{Standards}
	\gdef\@journalshort{Standards}
	\gdef\@doiabbr{standards}
	\gdef\@ISSN{2305-6703}	
	\gdef\@societyowner{}
}
\DeclareOption{stats}{%
	\gdef\@journal{stats}
	\gdef\@journalfull{Stats}
	\gdef\@journalshort{Stats}
	\gdef\@doiabbr{stats}
	\gdef\@ISSN{2571-905X}	
	\gdef\@societyowner{}
}
\DeclareOption{std}{%
	\gdef\@journal{std}
	\gdef\@journalfull{Surgical Techniques Development}
	\gdef\@journalshort{Surg. Tech. Dev.}
	\gdef\@doiabbr{std}
	\gdef\@ISSN{2038-9582}	
	\gdef\@societyowner{}
}
\DeclareOption{stresses}{%
	\gdef\@journal{stresses}
	\gdef\@journalfull{Stresses}
	\gdef\@journalshort{Stresses}
	\gdef\@doiabbr{stresses}
	\gdef\@ISSN{2673-7140}	
	\gdef\@societyowner{}
}
\DeclareOption{surfaces}{%
	\gdef\@journal{surfaces}
	\gdef\@journalfull{Surfaces}
	\gdef\@journalshort{Surfaces}
	\gdef\@doiabbr{surfaces}
	\gdef\@ISSN{2571-9637}	
	\gdef\@societyowner{}
}
\DeclareOption{surgeries}{%
	\gdef\@journal{surgeries}
	\gdef\@journalfull{Surgeries}
	\gdef\@journalshort{Surgeries}
	\gdef\@doiabbr{surgeries}
	\gdef\@ISSN{2017-2017}	
	\gdef\@societyowner{}
}
\DeclareOption{suschem}{%
	\gdef\@journal{suschem}
	\gdef\@journalfull{Sustainable Chemistry}
	\gdef\@journalshort{Sustain. Chem.}
	\gdef\@doiabbr{suschem}
	\gdef\@ISSN{2673-4079}	
	\gdef\@societyowner{}
}
\DeclareOption{sustainability}{%
	\gdef\@journal{sustainability}
	\gdef\@journalfull{Sustainability}
	\gdef\@journalshort{Sustainability}
	\gdef\@doiabbr{su}
	\gdef\@ISSN{2071-1050}
	\gdef\@societyowner{}
}
\DeclareOption{symmetry}{%
	\gdef\@journal{symmetry}
	\gdef\@journalfull{Symmetry}
	\gdef\@journalshort{Symmetry}
	\gdef\@doiabbr{sym}
	\gdef\@ISSN{2073-8994}
	\gdef\@societyowner{}
}
\DeclareOption{synbio}{%
	\gdef\@journal{synbio}
	\gdef\@journalfull{SynBio}
	\gdef\@journalshort{SynBio}
	\gdef\@doiabbr{synbio}
	\gdef\@ISSN{2674-0583}	
	\gdef\@societyowner{}
}
\DeclareOption{systems}{%
	\gdef\@journal{systems}
	\gdef\@journalfull{Systems}
	\gdef\@journalshort{Systems}
	\gdef\@doiabbr{systems}
	\gdef\@ISSN{2079-8954}
	\gdef\@societyowner{}
}
\DeclareOption{tae}{%
        \gdef\@journal{tae}
        \gdef\@journalfull{Theoretical and Applied Ergonomics}
        \gdef\@journalshort{Theor. Appl. Ergon.}
        \gdef\@doiabbr{tae}
        \gdef\@ISSN{}        
        \gdef\@societyowner{}
 }
\DeclareOption{targets}{%
	\gdef\@journal{targets}
	\gdef\@journalfull{Targets}
	\gdef\@journalshort{Targets}
	\gdef\@doiabbr{targets}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{taxonomy}{%
	\gdef\@journal{taxonomy}
	\gdef\@journalfull{Taxonomy}
	\gdef\@journalshort{Taxonomy}
	\gdef\@doiabbr{taxonomy}
	\gdef\@ISSN{2673-6500}	
	\gdef\@societyowner{}
}
\DeclareOption{technologies}{%
	\gdef\@journal{technologies}
	\gdef\@journalfull{Technologies}
	\gdef\@journalshort{Technologies}
	\gdef\@doiabbr{technologies}
	\gdef\@ISSN{2227-7080}
	\gdef\@societyowner{}
}
\DeclareOption{telecom}{%
	\gdef\@journal{telecom}
	\gdef\@journalfull{Telecom}
	\gdef\@journalshort{Telecom}
	\gdef\@doiabbr{telecom}
	\gdef\@ISSN{2673-4001}	
	\gdef\@societyowner{}
}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{Test}
	\gdef\@journalshort{Test}
	\gdef\@doiabbr{test}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{textiles}{%
	\gdef\@journal{textiles}
	\gdef\@journalfull{Textiles}
	\gdef\@journalshort{Textiles}
	\gdef\@doiabbr{textiles}
	\gdef\@ISSN{2673-7248}	
	\gdef\@societyowner{}
}
\DeclareOption{thalassrep}{%
	\gdef\@journal{thalassrep}
	\gdef\@journalfull{Thalassemia Reports}
	\gdef\@journalshort{Thalass. Rep.}
	\gdef\@doiabbr{thalassrep}
	\gdef\@ISSN{2039-4365}	
	\gdef\@societyowner{}
}
\DeclareOption{therapeutics}{%
	\gdef\@journal{therapeutics}
	\gdef\@journalfull{Therapeutics}
	\gdef\@journalshort{Therapeutics}
	\gdef\@doiabbr{therapeutics}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{thermo}{%
	\gdef\@journal{thermo}
	\gdef\@journalfull{Thermo}
	\gdef\@journalshort{Thermo}
	\gdef\@doiabbr{thermo}
	\gdef\@ISSN{2673-7264}	
	\gdef\@societyowner{}
}
\DeclareOption{timespace}{%
	\gdef\@journal{timespace}
	\gdef\@journalfull{Time and Space}
	\gdef\@journalshort{Time Space}
	\gdef\@doiabbr{timespace}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{tomography}{%
	\gdef\@journal{tomography}
	\gdef\@journalfull{Tomography}
	\gdef\@journalshort{Tomography}
	\gdef\@doiabbr{tomography}
	\gdef\@ISSN{2379-139X}	
	\gdef\@societyowner{}
}
\DeclareOption{tourismhosp}{%
	\gdef\@journal{tourismhosp}
	\gdef\@journalfull{Tourism and Hospitality}
	\gdef\@journalshort{Tour. Hosp.}
	\gdef\@doiabbr{tourhosp}
	\gdef\@ISSN{2673-5768}	
	\gdef\@societyowner{}
}
\DeclareOption{toxics}{%
	\gdef\@journal{toxics}
	\gdef\@journalfull{Toxics}
	\gdef\@journalshort{Toxics}
	\gdef\@doiabbr{toxics}
	\gdef\@ISSN{2305-6304}
	\gdef\@societyowner{}
}
\DeclareOption{toxins}{%
	\gdef\@journal{toxins}
	\gdef\@journalfull{Toxins}
	\gdef\@journalshort{Toxins}
	\gdef\@doiabbr{toxins}
	\gdef\@ISSN{2072-6651}
	\gdef\@societyowner{}
}
\DeclareOption{transplantology}{%
	\gdef\@journal{transplantology}
	\gdef\@journalfull{Transplantology}
	\gdef\@journalshort{Transplantology}
	\gdef\@doiabbr{transplantology}
	\gdef\@ISSN{2673-3943}	
	\gdef\@societyowner{}
}
\DeclareOption{transportation}{%
	\gdef\@journal{transportation}
	\gdef\@journalfull{Transportation}
	\gdef\@journalshort{Transportation}
	\gdef\@doiabbr{transportation}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{traumacare}{%
	\gdef\@journal{traumacare}
	\gdef\@journalfull{Trauma Care}
	\gdef\@journalshort{Trauma Care}
	\gdef\@doiabbr{traumacare}
	\gdef\@ISSN{2673-866X}	
	\gdef\@societyowner{}
}
\DeclareOption{traumas}{%
	\gdef\@journal{traumas}
	\gdef\@journalfull{Traumas}
	\gdef\@journalshort{Traumas}
	\gdef\@doiabbr{traumas}
	\gdef\@ISSN{2673-7477}	
	\gdef\@societyowner{}
}
\DeclareOption{tropicalmed}{%
	\gdef\@journal{tropicalmed}
	\gdef\@journalfull{Tropical Medicine and Infectious Disease}
	\gdef\@journalshort{Trop. Med. Infect. Dis.}
	\gdef\@doiabbr{tropicalmed}
	\gdef\@ISSN{2414-6366}
	\gdef\@societyowner{}
}
\DeclareOption{universe}{%
	\gdef\@journal{universe}
	\gdef\@journalfull{Universe}
	\gdef\@journalshort{Universe}
	\gdef\@doiabbr{universe}
	\gdef\@ISSN{2218-1997}
	\gdef\@societyowner{}
}
\DeclareOption{urbansci}{%
	\gdef\@journal{urbansci}
	\gdef\@journalfull{Urban Science}
	\gdef\@journalshort{Urban Sci.}
	\gdef\@doiabbr{urbansci}
	\gdef\@ISSN{2413-8851}
	\gdef\@societyowner{}
}
\DeclareOption{uro}{%
	\gdef\@journal{uro}
	\gdef\@journalfull{Uro}
	\gdef\@journalshort{Uro}
	\gdef\@doiabbr{uro}
	\gdef\@ISSN{2673-4397}	
	\gdef\@societyowner{}
}
\DeclareOption{vaccines}{%
	\gdef\@journal{vaccines}
	\gdef\@journalfull{Vaccines}
	\gdef\@journalshort{Vaccines}
	\gdef\@doiabbr{vaccines}
	\gdef\@ISSN{2076-393X}
	\gdef\@societyowner{}
}
\DeclareOption{vehicles}{%
	\gdef\@journal{vehicles}
	\gdef\@journalfull{Vehicles}
	\gdef\@journalshort{Vehicles}
	\gdef\@doiabbr{vehicles}
	\gdef\@ISSN{2624-8921}	
	\gdef\@societyowner{}
}
\DeclareOption{venereology}{%
	\gdef\@journal{venereology}
	\gdef\@journalfull{Venereology}
	\gdef\@journalshort{Venereology}
	\gdef\@doiabbr{venereology}
	\gdef\@ISSN{2674-0710}	
	\gdef\@societyowner{}
}
\DeclareOption{vetsci}{%
	\gdef\@journal{vetsci}
	\gdef\@journalfull{Veterinary Sciences}
	\gdef\@journalshort{Vet. Sci.}
	\gdef\@doiabbr{vetsci}
	\gdef\@ISSN{2306-7381}
	\gdef\@societyowner{}
}
\DeclareOption{vibration}{%
	\gdef\@journal{vibration}
	\gdef\@journalfull{Vibration}
	\gdef\@journalshort{Vibration}
	\gdef\@doiabbr{vibration}
	\gdef\@ISSN{2571-631X}	
	\gdef\@societyowner{}
}
\DeclareOption{virtualworlds}{%
	\gdef\@journal{virtualworlds}
	\gdef\@journalfull{Virtual Worlds}
	\gdef\@journalshort{Virtual Worlds}
	\gdef\@doiabbr{virtualworlds}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{viruses}{%
	\gdef\@journal{viruses}
	\gdef\@journalfull{Viruses}
	\gdef\@journalshort{Viruses}
	\gdef\@doiabbr{v}
	\gdef\@ISSN{1999-4915}
	\gdef\@societyowner{}
}
\DeclareOption{vision}{%
	\gdef\@journal{vision}
	\gdef\@journalfull{Vision}
	\gdef\@journalshort{Vision}
	\gdef\@doiabbr{vision}
	\gdef\@ISSN{2411-5150}
	\gdef\@societyowner{}
}
\DeclareOption{waste}{%
	\gdef\@journal{waste}
	\gdef\@journalfull{Waste}
	\gdef\@journalshort{Waste}
	\gdef\@doiabbr{waste}
	\gdef\@ISSN{2813-0391}	
	\gdef\@societyowner{}
}
\DeclareOption{water}{%
	\gdef\@journal{water}
	\gdef\@journalfull{Water}
	\gdef\@journalshort{Water}
	\gdef\@doiabbr{w}
	\gdef\@ISSN{2073-4441}
	\gdef\@societyowner{}
}
\DeclareOption{wem}{%
	\gdef\@journal{wem}
	\gdef\@journalfull{Wildlife Ecology and Management}
	\gdef\@journalshort{Wildl. Ecol. Manag.}
	\gdef\@doiabbr{wem}
	\gdef\@ISSN{1234-4321}
	\gdef\@societyowner{}
}
\DeclareOption{wevj}{%
	\gdef\@journal{wevj}
	\gdef\@journalfull{World Electric Vehicle Journal}
	\gdef\@journalshort{World Electr. Veh. J.}
	\gdef\@doiabbr{wevj}
	\gdef\@ISSN{2032-6653}
	\gdef\@societyowner{World Electric Vehicle Association}
}
\DeclareOption{wild}{%
	\gdef\@journal{wild}
	\gdef\@journalfull{Wild}
	\gdef\@journalshort{Wild}
	\gdef\@doiabbr{wild}
	\gdef\@ISSN{}	
	\gdef\@societyowner{}
}
\DeclareOption{wind}{%
	\gdef\@journal{wind}
	\gdef\@journalfull{Wind}
	\gdef\@journalshort{Wind}
	\gdef\@doiabbr{wind}
	\gdef\@ISSN{2674-032X}	
	\gdef\@societyowner{}
}
\DeclareOption{women}{%
	\gdef\@journal{women}
	\gdef\@journalfull{Women}
	\gdef\@journalshort{Women}
	\gdef\@doiabbr{women}
	\gdef\@ISSN{2673-4184}	
	\gdef\@societyowner{}
}
\DeclareOption{world}{%
	\gdef\@journal{world}
	\gdef\@journalfull{World}
	\gdef\@journalshort{World}
	\gdef\@doiabbr{world}
	\gdef\@ISSN{2673-4060}	
	\gdef\@societyowner{}
}
\DeclareOption{youth}{%
	\gdef\@journal{youth}
	\gdef\@journalfull{Youth}
	\gdef\@journalshort{Youth}
	\gdef\@doiabbr{youth}
	\gdef\@ISSN{2673-995X}	
	\gdef\@societyowner{}
}
\DeclareOption{zoonoticdis}{%
	\gdef\@journal{zoonoticdis}
	\gdef\@journalfull{Zoonotic Diseases}
	\gdef\@journalshort{Zoonotic Dis.}
	\gdef\@doiabbr{zoonoticdis}
	\gdef\@ISSN{2813-0227}	
	\gdef\@societyowner{}
}
